The Generative AI Paradox: "What It Can Create, It May Not Understand"

The recent wave of generative AI has sparked unprecedented global attention, with both excitement and concern over potentially superhuman levels of artificial intelligence: models now take only seconds to produce outputs that would challenge or exceed the capabilities even of expert humans. At the same time, models still show basic errors in understanding that would not be expected even in non-expert humans. This presents us with an apparent paradox: how do we reconcile seemingly superhuman capabilities with the persistence of errors that few humans would make? In this work, we posit that this tension reflects a divergence in the configuration of intelligence in today's generative models relative to intelligence in humans. Specifically, we propose and test the Generative AI Paradox hypothesis: generative models, having been trained directly to reproduce expert-like outputs, acquire generative capabilities that are not contingent upon -- and can therefore exceed -- their ability to understand those same types of outputs. This contrasts with humans, for whom basic understanding almost always precedes the ability to generate expert-level outputs. We test this hypothesis through controlled experiments analyzing generation vs. understanding in generative models, across both language and image modalities. Our results show that although models can outperform humans in generation, they consistently fall short of human capabilities in measures of understanding, as well as weaker correlation between generation and understanding performance, and more brittleness to adversarial inputs. Our findings support the hypothesis that models' generative capability may not be contingent upon understanding capability, and call for caution in interpreting artificial intelligence by analogy to human intelligence.

==> figures/collie_condensed_v2.tex <==
\begin{wrapfigure}{r}{0.58\textwidth}
% \vspace{-5pt}
\centering
% \includegraphics[width=\linewidth]{figures/language/collie_condensed_v2.pdf}
\includegraphics[width=\linewidth]{figures/language/collie_word1_sent24.pdf}
\vspace{-18pt}
\caption{GPT-4 Generative Constraint Satisfaction on Collie along with discriminative accuracy on its Generations. \ake{do we have human bars in here?}\faeze{no we assume human should have perfect acc on this. do you think we should put it in footnote?}\jena{It's in the text} \liwei{to be updated}}
% \vspace{-26pt}
\label{fig:gpt4_collie_condensed}
\end{wrapfigure}

==> figures/generation_example.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/generation_example.pdf}

    \caption{\peter{We will get a better example/figure, but start with this for a first draft} While GPT-4 generates a complete, novel, and well-formed story given a prompt, it fails to demonstrate an understanding of its own generation. In this case, it does not recognize (i) that it mentioned \emph{multiple sketches} drawn of the house and (ii) that the \emph{raw framework won't be exposed} when the house is nearly complete. Yet, the original generation does not contain such misunderstandings.}
    \label{fig:gen-example}
\end{figure}


==> figures/lang-expt2-main-results.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-4mm}
\centering
% \includegraphics[width=\linewidth]{figures/language/interrogative_exp2_vertical.pdf}
\includegraphics[width=\linewidth]{figures/language/interrogative_exp2_gpt4.pdf}
% \vspace{-15pt}
\caption{\small{Language: GPT-4 performance on generation and question answering based on its own output, versus human's performance on question answering based on GPT-4's output.}}
% \vspace{-26pt}
\label{fig:lang-expt2-main-results}
\end{wrapfigure}

==> figures/table_of_contents.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/table_of_contents.pdf}

    \caption{ \peter{This is a mockup, so section titles and ``Paradox?'' column won't be correct yet. Our main existing concerns besides this were: (i) should this be latex table? (ii) should we split experiments into 2 sections? Let me know if I missed anything from previous comments} \faeze{Great. I think we can convert it to latex for a more neat look and have line separator between "Understanding Type"/"Modality"/ etc. I can help with this:) }
    %\peter{Simple draft of the table of contents figure. Decided to do more of a dataframe format to try to capture comprehensiveness across multiple axes} \nouha{neat: should we convert it to latex, this is very low priority} \peter{I'm happy either way! Yejin has mentioned making a PDF to make it look cooler than a table, but I will admit that my current version isn't really leveraging this lol. I can make a second, latex table version in a while and we can decide (if we're alright with this format) \nouha{I'm happy either way too:)))}}\ximing{can we switch 3.2 and 3.3. I feel it makes more sense to first present exp1 (vision 3.1 and language 3.2) and then exp2 (vision 4.1 and languages 4.1).}\ximing{also for exp2 `understanding model's generation', we probe model with both selective (larger-scale) and descriptive (smaller-scale) evaluation, so maybe we can use another term to avoid confusion? such as "\textbf{interrogative}"}\faeze{interrogative sounds much better. Though I am still not sure if switching between modalities is ideal within a section and if having separate sections would make more sense. Like 3.1 and 3.2 for language exp1 and exp2 and similarly 4.1,4.2 for vision}} \peter{I agree about interrogative, and I have switched to using this in other places. Also happy to flip around section numbers and columns however we would like here. Will leave this for now as it's only a mock-up, and happy to switch it once we decide on final order (and on what should go in the ``Paradox'' column)
    }
    \label{fig:toc}
\end{figure}


==> sections/6_ethical_consideration.tex <==
\section{Limitations and Ethics}

\peter{I don't think ICLR requires this? We should still discuss limitations etc. but maybe in a smaller discussion section?}

\fb{authors are encouraged to include Ethics Statement}

==> sections/Jillians_thoughts_theory.tex <==
\textcolor{blue}{I agree that if you spend a whole section on theory of \textit{why} these paradox's are happening, you will need to show evidence for each of these points. I might just add it into section 2 or the discussion...}

\section{Paradox Theory}
We have identified three distinct features of language models which attribute to the paradoxes we have outlined. To speak more concretely, we use two representation models; the first is a traditional transformer language model $L$ and the second is an average adult human $H$.

\textcolor{blue}{ Maybe add a comment that says we can explain the LLM but not the human as well... do we have a cognitive psych person on the team?}

\paragraph{Knowledge and Training}  Each model is ``trained" on a training set, the language model $L$ is trained, using optimization of loss, on a large breadth of knowledge $x_{l}$, while the human $H$ has a less opaque learning process with a smaller training $x_h$. For large language models, we assume that $x_h \subset x_l$. 
\begin{enumerate}
    \item talk about how since $x_h \subset x_l$, LLM have more knowledge for generation. 
    \item Since LMM's optimization function is to maximize fluency (can add equation here), that is what they become good at --> i.e. generation
\end{enumerate}

\paragraph{Creation of Distributions}
When given an input $x$, the language model creates a distribution for the next token...
\begin{enumerate}
    \item talk about model representation learning and human information bottleneck 
    \item contrast with any theory about humans? 
\end{enumerate}

\paragraph{Choosing Next Token}
The language model $L$ is created to have a specific method for choosing the next token based on the distribution it creates. For example, at time step $t$ a model using greedy decoding uses,
\begin{align*}
    y_t = \argmax_{y\in V} P(y \vert y_1, y2,...,y_{t-1},x)
\end{align*}
\begin{enumerate}
    \item concrete, known selection process --> no judgement needed
    \item variation of distribution greatly affects humans (more variance, harder to choose), while it does not affect LM (it follows the decoding method)
\end{enumerate}



==> sections/history/2_hypotheses_v0.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/generation_understanding.png}
% \caption{[prototype] Generation and understanding for humans vs machines}
% \label{fig:prototype_sec2}
% % \vspace{-8pt}
% \end{figure}

% \nouha{Figure~\ref{fig:prototype_sec2}: (1) if humans can generate a correct response to a question, thus they can understand.
% (2) If humans can generate a correct response to a question, thus they can choose the correct response from a list of candidates (Demonstrated Understanding). 

% Human: (3) if we can select, it means we understand but that does not mean we can do generation. In certain contexts, humans may encounter difficulties when attempting to articulate their thoughts or generate text in response to a question.

% Understanding is necessary for generation but not sufficient.
% Understanding is sufficient and necessary for Demonstrated Understanding = selection

% Attaining the ability to select may imply the presence of understanding, but it is not enough to definitively assert this, because if generation occurs successfully, it signifies that understanding has taken place, and this is sufficient to enable selection.
% }\ximing{I feel 1) and 2) might be too strong, there can also be the case where a student simply memorize the answer from textbook without truly understand the knowledge. Teacher can identify this by asking them further question, or testing them through multiple choice exams} \nouha{very true .....}

\section{The Generative AI Paradox}


In this section, we begin by delving into the definitions of \textit{generation} and \textit{understanding} (\S\ref{subsec:definition}). Following this, we introduce the hypothesis of Generative AI Paradox and discuss the differing curvature of intelligence for humans and AIs when it comes to generating versus understanding (\S\ref{subsec:paradox}). Lastly, we explore methodologies for empirically testing our paradox hypothesis by probing understanding through \textit{selective} and \textit{interrogative} evaluation (\S\ref{subsec:testing_paradox}).
%\input{figures/table_of_contents}
\input{tables/table_of_content}
\subsection{Operational Definition of Generation and Understanding}
% \faeze{Maybe avoid having a section titled:ƒ Definition of Generation and Understanding, especially for Generation. Cannot think of a better title now but will think about it.}
% \yejin{we should say 'operational definitions' as opposed to 'definition', the latter is hard, while the former is up to us, thus more foregiving}\faeze{good idea!}
\label{subsec:definition}
We begin with properly defining the concept of \textit{generation} and \textit{understanding}. While several definitions have been proposed in computer and cognitive science fields, we choose to follow the most recent cogitative science literature. Here, the definition of generation and understanding applies to both humans and artificial intelligence. 

\textbf{Language Generation} is the process of producing a natural language text in order to achieve certain communicative objectives \citep{Dong2021ASO}. The generated texts may range from a brief response to a question, through multi-sentence comments and inquiries in a conversation, to comprehensive page-long descriptions. The goal of language generation is to produce effective language to foster reliable communication \citep{Moore2022LanguageMU}.
\textbf{Image Generation}
is the process of crafting realistic or stylized digital images that contain some particular desired content from textual inputs, sketches, or other images. 
Image generation can be exploited in various tasks such as inpainting, semantic scene synthesis, and super-resolution \citep{Zhang2023SurveyOC}. In this work, we focus on images generation from natural language descriptions. The goal of image generation is to produce high-quality images that faithfully represent the input descriptions.


\textbf{Understanding} is a cognitive activity of acquiring, integrating and expressing knowledge according to the task or situation at hand. The process of understanding can amount to an individual’s internal reflection on their own knowledge or abilities to accomplish a self-motivated goal \citep{Blaha2022UnderstandingIA}. \cite{Mahowald2023DissociatingLA} identifies four key capabilities required for understanding - formal reasoning, world knowledge, situation modeling, and social reasoning.  \jena{Mahowald paper's for capabilities listed are the key capabilies that allow language /use/, not just understanding.}

In summary, generation seeks to accomplish specific external goals, whereas understanding is an internal process that requires corresponding knowledge and reasoning capabilities.

\subsection{Generative AI Paradox}
\label{subsec:paradox}

Studies show that in humans, language understanding and production are complex cognitive skills that are intimately related \citep{clark1983comprehension, bock1996language}. A person's capability to produce relevant response depends upon one's capabilities to comprehend the context and question under discussion \citep{turgeon2008classical}. At the same time, the capability to appropriately understand the current context and situation also follows the prior experiences of successful production \citep{macdonald2013language, chater2016language}. %\nouha{I really like this!! Can we add citations}
%\jena{(explanation of the above: kids suck at the latter (they do comprehension better than production)... they end up saying stuff that are seemingly unrelated --- because they just lack experience/prior; also the case of aphasia shows that one can go broken and not the other. If soley the comprehension is broken, then you end up with fluent aphasia (they talk real well but intended meaning is incomprehensible); if the generation is broken then you end up with non-fluent or expressive aphasia where the person has trouble talking but produces appropriate meanings.}
%\jena{The funny bit is that language models are akin to fluent aphasia, but are able to produce sensical sentences -- ones that humans prefer over humans. Which is perplexing.}
Together they play a critical role in the larger cognitive functions that enable humans to abstract knowledge and experiences
%For humans, understanding serves as the cornerstone for generation, and paves the way to the robust use of language in the real world. Understanding enables human to abstract knowledge and 
experiences in order to make robust predictions, generalizations, and analogies, to reason compositionally and counterfactually, to actively intervene on the world in order to test hypotheses, and to explain one’s understanding to others \citep{Dong2021ASO, Goldwater2015OnTA, Gopnik2022CausalMA, Hofstadter2013SurfacesAE, Barrett2021ExplanationAU, Tenenbaum2018BuildingMT, Sloman2015CausalityIT, Smolensky2022NeurocompositionalCF}. Intuitively, a writer must undergo a complex thought process that involves establishing background, structuring the plot, and developing characters before crafting a novel, interesting story.  %\jena{establishing background and characters also require production not just comprehension?} 
\faeze{suggestion: According to cognitive process model of writing \citep{Flower1981}, writing (or composing) is best understood as a set of distinct hierarchical thinking processes which involves planning, translating, and reviewing. During the process of planning, writers combine information about the writing task with information from their long-term memory to generate a mental representation of the knowledge they will use in writing. %, and then they organize their ideas and set procedural and substantive goals in the form of a writing plan.
During the process of translating is when writers transform their mental representation into written language.} 

On the other hand, the relationship between understanding and generation is unclear for AI.
%It even remains unclear whether 
Its apparent behavior throws into question whether understanding is even a prerequisite for AI to produce successful generation.
Modern generative models, such as GPT-4 and Midjourney, display astonishing human-like generative capabilities, yet they are often subject to basic, persistent and unpredictable errors. For instance, GPT-4 exhibits human-level performance on various professional and academic benchmarks \citep{OpenAI2023GPT4TR}, yet it has been criticized for its lack of logical competence and ability to reason \citep{Arkoudas2023GPT4CR}. Similarly, while DALL-E produces stunning photorealistic images that far exceed the average human's drawing abilities, it still commits basic errors in areas like spatial relationships, object attributes, and object counting \citep{Cho2022DALLEvalPT}. 

We hypothesize that the inconsistencies in models' behavior suggests that the human \emph{curvature of intelligence} does not apply to models: while in humans capability to understand and use language are deeply interconnected, models follow a distinct, unpredictable curvature and progression, unintuitive to us. More concretely, we posit that models lack the interplay observed in human between production and comprehension, suggesting that the capability to \textit{generate} does not necessarily indicate the capability to \textit{understand}. 
In particular, we propose the \textbf{Generative AI Paradox}. Simply put,

\begin{tcolorbox}[boxrule=0.5pt,colback=white,arc=0mm, boxsep=-0.3mm]
\textbf{Hypothesis} \phantom{e}\textit{Models can produce impressive, genuinely useful \faeze{useful for what? looking for a better adj. how about "nearly flawless"?} \jena{or "seemingly flawless"} generations in modalities that they cannot demonstrate consistent \faeze{robust}, simple understanding of.}
\end{tcolorbox}


In words, this is saying the understanding of the model is significantly worse than what we expect from a human with the same generation capabilities.
%In the sections below, we'll assess to what extent the model acquires understanding capability when demonstrating impressive generation skills, and shed light on the reasons behind models' paradoxical behavior.

%\subsubsection{For AI, impressive generation ability does not premise robust understanding}


\jena{Thought for discussion: In humans, comprehension and production capabilities are interrelated with one another in such a way that generations can be employed to assess comprehension.} \ximing{agree}

\ximing{2.3.1, 2.3.2 done, ready to review}
\subsection{Evaluate Generation and Understanding Capabilities}
\label{subsec:testing_paradox}

To examine our hypothesis, we empirically evaluate to what extent generative AI possesses understanding capability when demonstrating impressive generation skills \faeze{we empirically evaluate the extent to which generative AI demonstrates understanding capability alongside its impressive generation skills}. The generation capability of a model is easily measurable by its success rate in fulfilling task requirements. However, assessing the model's understanding capability is less straightforward since we have no means\faeze{"no mean" is debatable especially from a mechanistic interpretability perspective} to access its internal representation or reasoning procedures. Taking inspiration from human cognitive processes \faeze{is there any citation on this?}, we propose using \textit{selective} and \textit{interrogative} probings as indicators to estimate the model's understanding capability.  We will begin with a few preliminaries on generative AI.

%While generation capability can be simply measured by the success rate for model's generation to meet task requirement, how to evaluate understanding capability is less obvious as we have no means to access model's internal representation and reasoning procedure. Drawing inspirations from the cognitive procedure of human, we propose selective and interrogative probings as indicators to estimate model's understanding capability. We will first start with some preliminaries of generative models. 
% To test our hypothesis, we empirically evaluate the extent to which the model demonstrates an understanding capability alongside its impressive generative skills. The generation capability of a model is easily measurable by its success rate in fulfilling task requirements. However, assessing its understanding capability is less straightforward since we don't have means to access the model's internal representation and reasoning procedures. Taking inspiration from human cognitive processes, we propose using selective and interrogative probings as markers to estimate the understanding capability of the model. We will begin with a few preliminaries on generative models.
\subsubsection{Preliminaries of Generative AI}

\faeze{I think we can skip this preliminaries as we dicuss these details in the exp section. wdut?} \ximing{alternatively we can skip all the details in experiment? I feel it might be helpful to give an overview early in the paper, especially for saying people in NLP who's not familiar with how vision works.}
In language domain, it is the common practice is to have a unified language model $M$ (e.g. GPT-4) for all tasks and applications, which generates output text $\textbf{y}$ from an input text prompt $\textbf{x}$.

On the other hand, we have distinct models in vision domain. For image generation, we have a specialized generative model $M_G$ (e.g. DALL-E) which produces an image $\textbf{I}_y$ that corresponds to the input textual caption $\textbf{x}$. For general vision-language (VL) tasks such as visual question answering, we have a general-purpose VL model $M_D$ (e.g. BLIP-2) that outputs a text response $\textbf{y}$, in answer to the input text query $\textbf{x}$ based on the information from the input image $\textbf{I}_x$. Here, we consider discriminative VL models such as CLIP to be a special case of the general-purpose VL models which output a Boolean value $\textbf{y}$ to indicate if the input image $\textbf{I}_x$ corresponds to the input caption $\textbf{x}$.

%On the other hand, in vision domain, there are separate image generative model $M_G$ (e.g. DALL-E) and general-purpose vision-language model $M_D$ (e.g. BLIP-2, Bard) for image generation and solving vision-language tasks respectively. 

\subsubsection{Probe understanding as selection}
With a genuine understanding, it would be easier for humans to distinguish between correct and incorrect responses compared to generate the correct response \faeze{$\leftarrow$ I think by now we made this point clear. Also next sentence kind of say the same thing. how about removing the first sentence?} \ximing{sounds good}. Human often intuitively prefer multiple-choice questions and perform better on them compared to open-ended ones \cite{funkanddickson}. Inspired by this, we investigate whether a generative model, when capable of producing the correct answer in an open-ended format, can also consistently choose the correct option in a multiple-choice setting. Specifically, we assess the model's performance on identical tasks in both multiple-choice and open-ended formats, and then compare this to human performance in the same contexts. Formally, we denote the generative and discriminative accuracy of an agent as follows:
    \begin{align*}
    \small
        \text{Acc}_G(P_\theta) = \frac{\sum_{\textbf{x} \sim \mathcal{D}}\mathbbm{1}(\textbf{y} \in \hat{Y}), \textbf{y} \sim {P_\theta(\textbf{y}|\textbf{x})}}{\|\mathcal{D}\|}, \: \text{Acc}_D(P_\theta) = \frac{\sum_{(\textbf{x}, \hat{\textbf{y}}, C) \sim \mathcal{D}}\mathbbm{1}\big(\arg\max P_\theta(\textbf{y} | \textbf{x}, C) = \hat{\textbf{y}} \big)}{\|\mathcal{D}\|}
    \end{align*}
Here, $\theta$ represents an agent that can be either a model or a human. $\mathcal{D}$ denotes the test set for a specific task, $C$ denotes the set of candidates for a given query $\textbf{x}$. $\hat{\textbf{y}}$ is the ground-truth response, and $\hat{Y}$ represents the set of acceptable answers. In practice, we use human evaluation to determine if a generated response falls within the acceptable set.

For language, we use the unified model $M$ for both generation and selection. We explore a wide range of language-related tasks, such as dialogue, conversational QA, general QA, summarization, and commonsense reasoning. 
For tasks originally in multiple-choice format, like CSQA, we transformed them into generative tasks by omitting the candidates. 
Conversely, for tasks initially in a generative format, such as summarization, we changed them to multiple-choice by creating incorrect candidates.
We did this by perturbing the groundtruth response, for instance by introducing hallucinations. By adjusting the similarity between the incorrect and correct options, we can vary the difficulty of the multiple-choice task.

For vision, we use the generative model $M_G$ for image generation, and the general-purpose vision model $M_D$ for selection. Superficially, we prompt $M_G$ to generate images given the text descriptions, and ask $M_D$ to select the image, that better matches the text description from candidates.


\subsubsection{Probe understanding as interrogation}
With genuine understanding, a human would be able to answer basic questions about their own generation. Indeed, in oral exams, it's common to ask a series of questions based on prior answers to gauge a student's grasp of the subject. Similarly, we assess if a model can demonstrate a meaningful understanding of its own outputs by posing questions based on its own generated content. Concretely, we evaluate the model's question-answering performance given its own generated content as context. Formally,
    \begin{align*}
    \small
        \text{Acc}_U(P_\theta) = \frac{\sum_{\textbf{x} \sim \mathcal{D}}\mathbbm{1}(\textbf{r} \in \hat{R}), \textbf{r} \sim {P_\theta(\textbf{r}|\textbf{y})}, \textbf{y} \sim {P_\theta(\textbf{y}|\textbf{x})}}{\|\mathcal{D}\|}
    \end{align*}
For language, we first ask models to generate a paragraph-level text while taking into account some background information. We then ask model to use its generated content to answer background-related questions. For vision, we first prompt $M_G$ to generate images given the text descriptions, and then ask $M_D$ to answer questions about the content of these generated images.






%\ximing{note below, ignore}

%3 points we discussed:
%Discuss understanding and discrimination. 
%Notes from Yejin:
%ection 2: Overview table + list of observations

%\begin{enumerate}
%\item start by comparing humans vs AI in the intro: put forward the generative AI paradox which means Bla
%\item Intro: humans are worse than machines in generating impressive text. 
%\item the current situation raises the generative AI paradox:
%\item in this paper, provide news insights and reasons as to why these are the case: distractors and nature of the tasks, IID vs OOD 
%\item the goal is to shed light on the difference between AI intelligence and human intelligence. 
%\item compare LLMs in discrimination setup vs generation setup
%\item there are several dimensions for understanding 
%\item Compare human performance in discrimination and generation vs humans
%\item D
%\item organize different cases: what it means to understand:
%\item Different cells 

%A few more notes from Yejin:
%\begin{enumerate}
%    \item result is not binary
%    \item "in this paper we aim to answer this question by developing different formulation of the problem"
%    \item "curvature of intelligence in AI is more convoluted than expected"
%    \item "their curvature is highly fluctuating"
%    \item what people should cite us for: (1) "AI is not black magic in all dimensions" (2) generative AI and its limitations
%    \item use very low-key, plain language
%    \item make it more about asking questions
%    \item tone down the argument and it will have impact
%\end{enumerate}

%\item 


%\end{enumerate}

% Peter's comments:
% \begin{enumerate}
%     \item I really agree with how we framed what models are doing, although we will probably need to be careful about exactly how we state this in the paper. e.g. I do think comparative reasoning highlights why they fail, although there probably aren’t any universal breaks (like the elimination example) so we may need to be somewhat subtle/vague if and when we state this idea in the paper
% \item Likewise, really agree with thoughts about humans, but I’m guessing we’ll need to be fairly subtle/rely on reader commonsense for some of this, as there is still quite a bit of disagreement ito how humans learn and reason, and we don’t want to get caught in that debate
% \item I don’t think either above point means we should do things differently, just that we’ll need to be careful, and plan to do followup work where we might make stronger statements e.g. to do a more comprehensive empirical study of why the paradox happens, where I’m guessing we’ll need to spend more space in this paper simply proving that it happens at all
% \end{enumerate}

$ $

breif operationized definition
see appendix for comprehensive literature



\section{(Peter's outline \S2, if it may be useful) Overview: The Generative AI Paradox}

\peter{Ignore the version below. I was thinking of writing a much shorter version but will not for now unless we need it.}

First, we provide an overview of the Generative AI Paradox. % \peter{Need a better first sentence to describe what this section is for}
Beginning with a case study (\S\ref{subsec:case-study}), we develop intuitions for the generation-understanding gap in generative AI, which are then developed into definitions and a complete statement of the paradox (\S\ref{subsec:definitions}). Finally, we present an overview of the remainder of the paper (\S\ref{subsec:overview}).

\subsection{Case Study: Can LMs understand their own generations?}
\label{subsec:case-study}

To gain intuition for how models generate and understand, we begin with a short case study. We prompt GPT-4 to \emph{Write a two paragraph story about 3 people building a house}, with an abridged version of this story in Figure~\ref{fig:gen-example} and the full story included in the Appendix. While artistic merit could be debated, the story fully satisfies the prompt, including details about the ``breathtaking design of a two-storied country house'' and how the 3 people would ``sit together on the raw framework, overlooking green hills, discussing the interior decoration'' on breaks between building the house. We could find no obvious faults with the story.

Next, we ask GPT-4 a series of simple, natural questions about its own story to gauge its understanding. Intuitively, we expect a human capable of generating such a story to correctly answer questions about it, but the behavior of GPT-4 was not so straightforward. When asked how many designs were sketched, GPT-4 says only 1, despite mentioning years of previous designs. When asked what the 3 did on the \emph{final} break before finishing the house, it still says they sat on the ``raw framework'' of the house, which would almost certainly not be exposed by that point in construction. 

Surprisingly, the ability of GPT-4 to understand the story does not seem to match the model's ability to generate it. The generation itself does not seem to imply any of the errors, and also seems to be novel--we could not find significant overlap with data on the web. This case study poses a mystery: \emph{Could GPT-4 really generate a novel, quality story that it does not itself seem to understand?}
%\nouha{These paragraphs are really great but I think they're telling a preview of what we will discuss in exp 2. We can summarize them and include the example in intro, no?}
%\peter{Could definitely move it, but I do think one thing that's kind of missing is a clear example of the paradox that people can point at/identify with. We kind of allude to this in the intro, but probably don't take enough time for it to be obvious/intuitive to people imo. But this could also be something like the way people use vision models (which is what Yejin always uses as an obvious example) but then this is just kind of exp 1 instead I guess?}. \nouha{Agreed! we definitely need nice examples, I think we should include a vision example in the same figure to show the paradox from both modalities. For example, we can show only one failure case for language and remove the other question. Condense the GPT4 paragraph to have room for the vision obvious example. wdyt? I'm fine with this too} \peter{I do like the idea of one example each -- this makes it a lot easier to explain both (i) the two different settings (selective and interrogative) and very quickly make it clear that we do 2 modalities. Anyhow, I'll think about how to reorganize this figure if we're thinking about using this idea (vs sticking to what Ximing has above)}

\subsection{Definitions and Paradox}

\label{subsec:def-and-paradox}

In order to pose this idea formally and experimentally, we draw out the boundaries and definitions of what we will be studying here.

While our case study above focuses on language, this mismatch between generation and understanding seems to apply to generative models across modalities. One example is the emergent mode-of-use for image generators like Midjourney (CITE): the model produces multiple image candidates, which the human user then chooses between. In effect, humans are delegating the seemingly harder generation task, while doing the easier task of selection (understanding). Thus, we would like to pose our study for generative models \textbf{across modalities}, in this work for vision and language specifically.

The GPT-4 case study and mode-of-use for Midjourney draw out \textbf{2 strong yet distinct methods by which understanding is typically tested}:
\begin{enumerate}
    \item \textbf{Selective evaluation} in which understanding is demonstrated by evaluating whether objects fit a given query. Multiple choice question answering is one clear example, which is one of the most common ways to examine human understanding (CITE), as well as natural language understanding in language models (CITE). The mode-of-use of Humans picking between different Midjourney outputs fits this method.
    \item \textbf{Interrogative evaluation} in which understanding is tested with a series of probing questions to draw out the overall understanding of a document by some agent. The case study above fits this method, which is similar to oral exams that students take.
\end{enumerate}
We conduct experiments following both of these styles. We focus on ways understanding is \emph{evaluated or expressed} rather than its underlying definition, which is difficult or impossible to experimentally verify. \nouha{Not sure if we should say "outloud" that defining understanding is difficult or impossible hehe} However, we note that selective and interrogative evaluation fit previous theoretical definitions from epistemology (CITE Karavig), respectively (1) propositional understanding, which is the understanding of the correctness of one statement like "item X satisfies statement Y" and (2) objectual understanding, which is understanding of complete objects ("I understand image Z") which may be encompass many individual pieces of knowledge. 

Yet another factor in studying AI understanding and generation is \textbf{whether the same model is for both}. We study both the case where the models are identical, and where they are different (as is common in the vision domain).

As mentioned above, the reason the behavior of GPT-4 seems contradictory in this case study, is that we would expect a \emph{human} capable of generating such a story to understand their own generation, and be able to demonstrate that understanding. Thus, we will broadly \textbf{frame our work here through the capabilities of humans}, the only systems previously able to produce content of this quality. A broad, implicit hypothesis raised by past work (CITE CITE) is that this similar ability to generate content implies similar forms of intelligence between humans and models; the case study above does not support this, and leads to a statemenet of our hypothesis, the \textbf{Generative AI Paradox:}

\begin{displayquote}

\emph{While generative models produce impressive, useful generations across modalities, they do not demonstrate the simple, consistent understanding we would expect of humans with the same capabilities.}

\end{displayquote}

In mathematical terms, we can state this loosely as:

$$ U_{human | G_{model}} - U_{model} > \epsilon $$

Where, for a given task, $U_{model}$ is the evaluated model understanding performance, $G_{model}$ is the evaluated model generation performance, $U_{human | G_{model}}$ is the human understanding performance we would expect given the capacity to generate at the level of the model, and $\epsilon$ is some constant representing a significant difference.

In words, this is saying the understanding of the model $U_{model}$ is significantly worse than what we expect from a human with the same generation capabilities $U_{human | G_{model}}$. It is not clear if this is true in every setting, but in the two examples so far, it seems to be. In using Midjourney, humans who are not even capable of generating images can still complete the understanding take, which models struggle with (so in this case, we take average human understanding to lowerbound the understanding a human capable of the generation task would have). In the case study above, we make the fairly straightforward assumption that any human who can generate the given story will be able to answer these questions nearly perfectly, while the model fails. 

\peter{Probably elaborate on why this is interesting a bit more.}
\nouha{This is great. We will have to condense it and merge it with the previous paragraphs.  }
\peter{agreed! I probably should have mentioned (and this is relevant to earlier parts) -- I was mainly trying to maximize clarity without thinking too much about length, with the intention of hyper-compressing if we end up using anything. But more just looking to figure out what we might want to say in as clear terms as possible} \nouha{yup, we need to really condense}
\subsection{Roadmap}

Given the definitions above, we finally lay out a road map for the rest of the paper.

\S? - \S? begin by carrying out a comprehensive range of experiments covering the factors in \S\ref{subsec:def-and-paradox}. Refer to Figure~\ref{fig:toc} for modelity, understanding type, and whether the generator is the same as the understanding model are covered in these experiments. 

Next, \S? discusses when and how our results support the existence of this paradox. We find a subtle and complex story, but generally verify that this contradiction is real in a range of controlled settings.

\S? then discusses a range of proposals for \emph{why} this may be the case, ranging from ... 

Finally, \S? discusses the limitations of the current work, and what we propose future work should consider. We finish the paper with related work (\S?) and overall conclusions (\S?).

==> sections/history/2_hypotheses_v1.tex <==
\section{The Generative AI Paradox}



\peter{Following Yejin's suggestion, pushing this version up to S2. }
\peter{DO NOT LOOK AT CURRENT VERSION YET! I will shorten and improve this tomorrow (Tuesday) morning, and ping the main channel when done.}
%\ximing{I thought what yejin means is to push the current \textbf{experiments section} as section 2, and merge with the original section we have. I got a bit confused, I've pinged the channel to confirm}

\input{tables/table_of_content}


First, we provide an overview of the Generative AI Paradox. % \peter{Need a better first sentence to describe what this section is for}
Beginning with a case study (\S\ref{subsec:case-study}), we develop intuitions for the generation-understanding gap in generative AI, which are then developed into definitions and a complete statement of the paradox (\S\ref{subsec:definitions}). Finally, we present an overview of the remainder of the paper (\S\ref{subsec:overview}).

\subsection{Case Study: Can LMs understand their own generations?}
\label{subsec:case-study}

To gain intuition for how models generate and understand, we begin with a short case study. We prompt GPT-4 to \emph{Write a two paragraph story about 3 people building a house}, with an abridged version of this story in Figure~\ref{fig:gen-example} and the full story included in the Appendix. While artistic merit could be debated, the story fully satisfies the prompt, including details about the ``breathtaking design of a two-storied country house'' and how the 3 people would ``sit together on the raw framework, overlooking green hills, discussing the interior decoration'' on breaks between building the house. We could find no obvious faults with the story.

Next, we ask GPT-4 a series of simple, natural questions about its own story to gauge its understanding. Intuitively, we expect a human capable of generating such a story to correctly answer questions about it, but the behavior of GPT-4 was not so straightforward. When asked how many designs were sketched, GPT-4 says only 1, despite mentioning years of previous designs. When asked what the 3 did on the \emph{final} break before finishing the house, it still says they sat on the ``raw framework'' of the house, which would almost certainly not be exposed by that point in construction. 

Surprisingly, the ability of GPT-4 to understand the story does not seem to match the model's ability to generate it. The generation itself does not seem to imply any of the errors, and also seems to be novel--we could not find significant overlap with data on the web. This case study poses a mystery: \emph{Could GPT-4 really generate a novel, quality story that it does not itself seem to understand?}
%\nouha{These paragraphs are really great but I think they're telling a preview of what we will discuss in exp 2. We can summarize them and include the example in intro, no?}
%\peter{Could definitely move it, but I do think one thing that's kind of missing is a clear example of the paradox that people can point at/identify with. We kind of allude to this in the intro, but probably don't take enough time for it to be obvious/intuitive to people imo. But this could also be something like the way people use vision models (which is what Yejin always uses as an obvious example) but then this is just kind of exp 1 instead I guess?}. \nouha{Agreed! we definitely need nice examples, I think we should include a vision example in the same figure to show the paradox from both modalities. For example, we can show only one failure case for language and remove the other question. Condense the GPT4 paragraph to have room for the vision obvious example. wdyt? I'm fine with this too} \peter{I do like the idea of one example each -- this makes it a lot easier to explain both (i) the two different settings (selective and interrogative) and very quickly make it clear that we do 2 modalities. Anyhow, I'll think about how to reorganize this figure if we're thinking about using this idea (vs sticking to what Ximing has above)}

\subsection{Paradox and Operational Definitions}

\label{subsec:def-and-paradox}

In order to pose this idea formally and experimentally, we draw out the boundaries and definitions of what we will be studying here.

While our case study above focuses on language, this mismatch between generation and understanding seems to apply to generative models across modalities. One example is the emergent mode-of-use for image generators like Midjourney (CITE): the model produces multiple image candidates, which the human user then chooses between. In effect, humans are delegating the seemingly harder generation task, while doing the easier task of selection (understanding). Thus, we would like to pose our study for generative models \textbf{across modalities}, in this work for vision and language specifically.

The GPT-4 case study and mode-of-use for Midjourney draw out \textbf{2 strong yet distinct methods by which understanding is typically tested}:
\begin{enumerate}
    \item \textbf{Selective evaluation} in which understanding is demonstrated by evaluating whether objects fit a given query. Multiple choice question answering is one clear example, which is one of the most common ways to examine human understanding (CITE), as well as natural language understanding in language models (CITE). The mode-of-use of Humans picking between different Midjourney outputs fits this method.
    \item \textbf{Interrogative evaluation} in which understanding is tested with a series of probing questions to draw out the overall understanding of a document by some agent. The case study above fits this method, which is similar to oral exams that students take.
\end{enumerate}
We conduct experiments following both of these styles. We focus on ways understanding is \emph{evaluated or expressed} rather than its underlying definition, which is difficult or impossible to experimentally verify. \nouha{Not sure if we should say "outloud" that defining understanding is difficult or impossible hehe} However, we note that selective and interrogative evaluation fit previous theoretical definitions from epistemology (CITE Karavig), respectively (1) propositional understanding, which is the understanding of the correctness of one statement like "item X satisfies statement Y" and (2) objectual understanding, which is understanding of complete objects ("I understand image Z") which may be encompass many individual pieces of knowledge. 

Yet another factor in studying AI understanding and generation is \textbf{whether the same model is for both}. We study both the case where the models are identical, and where they are different (as is common in the vision domain).

As mentioned above, the reason the behavior of GPT-4 seems contradictory in this case study, is that we would expect a \emph{human} capable of generating such a story to understand their own generation, and be able to demonstrate that understanding. Thus, we will broadly \textbf{frame our work here through the capabilities of humans}, the only systems previously able to produce content of this quality. A broad, implicit hypothesis raised by past work (CITE CITE) is that this similar ability to generate content implies similar forms of intelligence between humans and models; the case study above does not support this, and leads to a statemenet of our hypothesis, the \textbf{Generative AI Paradox:}

\begin{displayquote}

\emph{While generative models produce impressive, useful generations across modalities, they do not demonstrate the simple, consistent understanding we would expect of humans with the same capabilities.}

\end{displayquote}

In mathematical terms, we can state this loosely as:

$$ U_{human | G_{model}} - U_{model} > \epsilon $$

Where, for a given task, $U_{model}$ is the evaluated model understanding performance, $G_{model}$ is the evaluated model generation performance, $U_{human | G_{model}}$ is the human understanding performance we would expect given the capacity to generate at the level of the model, and $\epsilon$ is some constant representing a significant difference.

In words, this is saying the understanding of the model $U_{model}$ is significantly worse than what we expect from a human with the same generation capabilities $U_{human | G_{model}}$. It is not clear if this is true in every setting, but in the two examples so far, it seems to be. In using Midjourney, humans who are not even capable of generating images can still complete the understanding take, which models struggle with (so in this case, we take average human understanding to lowerbound the understanding a human capable of the generation task would have). In the case study above, we make the fairly straightforward assumption that any human who can generate the given story will be able to answer these questions nearly perfectly, while the model fails. 

\peter{Probably elaborate on why this is interesting a bit more.}
\nouha{This is great. We will have to condense it and merge it with the previous paragraphs.  }
\peter{agreed! I probably should have mentioned (and this is relevant to earlier parts) -- I was mainly trying to maximize clarity without thinking too much about length, with the intention of hyper-compressing if we end up using anything. But more just looking to figure out what we might want to say in as clear terms as possible} \nouha{yup, we need to really condense}
\subsection{Roadmap}

Given the definitions above, we finally lay out a road map for the rest of the paper.

\S? - \S? begin by carrying out a comprehensive range of experiments covering the factors in \S\ref{subsec:def-and-paradox}. Refer to Figure~\ref{fig:toc} for modelity, understanding type, and whether the generator is the same as the understanding model are covered in these experiments. 

Next, \S? discusses when and how our results support the existence of this paradox. We find a subtle and complex story, but generally verify that this contradiction is real in a range of controlled settings.

\S? then discusses a range of proposals for \emph{why} this may be the case, ranging from ... 

Finally, \S? discusses the limitations of the current work, and what we propose future work should consider. We finish the paper with related work (\S?) and overall conclusions (\S?).




\section{The Generative AI Paradox}

In this section, we begin by delving into the definitions of \textit{generation} and \textit{understanding} (\S\ref{subsec:definition}). Following this, we introduce the hypothesis of Generative AI Paradox and discuss the differing curvature of intelligence for humans and AIs when it comes to generating versus understanding (\S\ref{subsec:paradox}). Lastly, we explore methodologies for empirically testing our paradox hypothesis by probing understanding through \textit{selective} and \textit{interrogative} evaluation (\S\ref{subsec:testing_paradox}).
%\input{figures/table_of_contents}

\subsection{Operational Definition of Generation and Understanding}
% \faeze{Maybe avoid having a section titled: Definition of Generation and Understanding, especially for Generation. Cannot think of a better title now but will think about it.}
% \yejin{we should say 'operational definitions' as opposed to 'definition', the latter is hard, while the former is up to us, thus more foregiving}\faeze{good idea!}
\label{subsec:definition}
Several definitions have been proposed in computer and cognitive science fields that define the concepts of \textit{generation} and \textit{understanding}. In this section, we begin by providing high-level definitions for the terms as operalizationalized in the present investigation. 
%While several definitions have been proposed in computer and cognitive science fields, we choose to follow the most recent cogitative science literature. Here, the definition of generation and understanding applies to both humans and artificial intelligence. 

\textbf{Language Generation} is the process of producing comprehensible natural language text that achieves the purpose of relaying on the a message in an effective manner \citep{Dong2021ASO, Moore2022LanguageMU}. We experiment with varying types of generations ranging from short responses to questions to open-ended paragraph completions.
%\textbf{Language Generation} is the process of producing a natural language text in order to achieve certain communicative objectives \citep{Dong2021ASO}. The generated texts may range from a brief response to a question, through multi-sentence comments and inquiries in a conversation, to comprehensive page-long descriptions. The goal of language generation is to produce effective language to foster reliable communication \citep{}.
%
\textbf{Image Generation}
is the process of crafting realistic or stylized digital images that contain some particular desired content,
%from textual inputs, sketches, or other images. 
and has been exploited in various tasks such as inpainting, semantic scene synthesis, and super-resolution \citep{Zhang2023SurveyOC}. In this work, we focus on images generation from natural language descriptions. The goal of image generation is to produce high-quality images that faithfully represent the input descriptions.

\textbf{Understanding} refers to the mental activity of grasping or making sense of a message or information presented  \citep{Blaha2022UnderstandingIA}. 
%is a cognitive activity of acquiring, integrating and expressing knowledge according to the task or situation at hand. 
%In humans, the process of understanding incorporates both the
%The process of understanding can amount to an individual’s internal reflection on their own knowledge or abilities to accomplish a self-motivated goal
\cite{Mahowald2023DissociatingLA} identifies four key capabilities required for understanding - formal reasoning, world knowledge, situation modeling, and social reasoning.  \jena{Mahowald paper's for capabilities listed are the key capabilies that allow language /use/, not just understanding.}

%In summary, generation seeks to accomplish specific external goals, whereas understanding is an internal process that requires corresponding knowledge and reasoning capabilities. \jena{This is far to simplistic a view... }

\subsection{Generative AI Paradox}
\label{subsec:paradox}

Studies show that in humans, language understanding and production are complex cognitive skills that are intimately related \citep{clark1983comprehension, bock1996language}. A person's capability to produce relevant response depends upon one's capabilities to comprehend the context and question under discussion \citep{turgeon2008classical}. At the same time, the capability to appropriately understand the current context and situation also follows the prior experiences of successful production \citep{macdonald2013language, chater2016language}. %\nouha{I really like this!! Can we add citations}
%\jena{(explanation of the above: kids suck at the latter (they do comprehension better than production)... they end up saying stuff that are seemingly unrelated --- because they just lack experience/prior; also the case of aphasia shows that one can go broken and not the other. If soley the comprehension is broken, then you end up with fluent aphasia (they talk real well but intended meaning is incomprehensible); if the generation is broken then you end up with non-fluent or expressive aphasia where the person has trouble talking but produces appropriate meanings.}
%\jena{The funny bit is that language models are akin to fluent aphasia, but are able to produce sensical sentences -- ones that humans prefer over humans. Which is perplexing.}
Together they play a critical role in the larger cognitive functions that enable humans to abstract knowledge and experiences
%For humans, understanding serves as the cornerstone for generation, and paves the way to the robust use of language in the real world. Understanding enables human to abstract knowledge and 
experiences in order to make robust predictions, generalizations, and analogies, to reason compositionally and counterfactually, to actively intervene on the world in order to test hypotheses, and to explain one’s understanding to others \citep{Dong2021ASO, Goldwater2015OnTA, Gopnik2022CausalMA, Hofstadter2013SurfacesAE, Barrett2021ExplanationAU, Tenenbaum2018BuildingMT, Sloman2015CausalityIT, Smolensky2022NeurocompositionalCF}. Intuitively, a writer must undergo a complex thought process that involves establishing background, structuring the plot, and developing characters before crafting a novel, interesting story.  %\jena{establishing background and characters also require production not just comprehension?} 
\faeze{suggestion: According to cognitive process model of writing \citep{Flower1981}, writing (or composing) is best understood as a set of distinct hierarchical thinking processes which involves planning, translating, and reviewing. During the process of planning, writers combine information about the writing task with information from their long-term memory to generate a mental representation of the knowledge they will use in writing. %, and then they organize their ideas and set procedural and substantive goals in the form of a writing plan.
During the process of translating is when writers transform their mental representation into written language.} 

On the other hand, the relationship between understanding and generation is unclear for AI.
%It even remains unclear whether 
Its apparent behavior throws into question whether understanding is even a prerequisite for AI to produce successful generation.
Modern generative models, such as GPT-4 and Midjourney, display astonishing human-like generative capabilities, yet they are often subject to basic, persistent and unpredictable errors. For instance, GPT-4 exhibits human-level performance on various professional and academic benchmarks \citep{OpenAI2023GPT4TR}, yet it has been criticized for its lack of logical competence and ability to reason \citep{Arkoudas2023GPT4CR}. Similarly, while DALL-E produces stunning photorealistic images that far exceed the average human's drawing abilities, it still commits basic errors in areas like spatial relationships, object attributes, and object counting \citep{Cho2022DALLEvalPT}. 

We hypothesize that the inconsistencies in models' behavior suggests that the human \emph{curvature of intelligence} does not apply to models: while in humans capability to understand and use language are deeply interconnected, models follow a distinct, unpredictable curvature and progression, unintuitive to us. More concretely, we posit that models lack the interplay observed in human between production and comprehension, suggesting that the capability to \textit{generate} does not necessarily indicate the capability to \textit{understand}. 
In particular, we propose the \textbf{Generative AI Paradox}. Simply put,

\begin{tcolorbox}[boxrule=0.5pt,colback=white,arc=0mm, boxsep=-0.3mm]
\textbf{Hypothesis} \phantom{e}\textit{Models can produce impressive, genuinely useful \faeze{useful for what? looking for a better adj. how about "nearly flawless"?} \jena{or "seemingly flawless"} generations in modalities that they cannot demonstrate consistent \faeze{robust}, simple understanding of.}
\end{tcolorbox}


In words, this is saying the understanding of the model is significantly worse than what we expect from a human with the same generation capabilities.
%In the sections below, we'll assess to what extent the model acquires understanding capability when demonstrating impressive generation skills, and shed light on the reasons behind models' paradoxical behavior.

%\subsubsection{For AI, impressive generation ability does not premise robust understanding}


\jena{Thought for discussion: In humans, comprehension and production capabilities are interrelated with one another in such a way that generations can be employed to assess comprehension.} \ximing{agree}

\ximing{2.3.1, 2.3.2 done, ready to review}
\subsection{Evaluate Generation and Understanding Capabilities}
\label{subsec:testing_paradox}

To examine our hypothesis, we empirically evaluate to what extent generative AI possesses understanding capability when demonstrating impressive generation skills \faeze{we empirically evaluate the extent to which generative AI demonstrates understanding capability alongside its impressive generation skills}. The generation capability of a model is easily measurable by its success rate in fulfilling task requirements. However, assessing the model's understanding capability is less straightforward since we have no means\faeze{"no mean" is debatable especially from a mechanistic interpretability perspective} to access its internal representation or reasoning procedures. Taking inspiration from human cognitive processes \faeze{is there any citation on this?}, we propose using \textit{selective} and \textit{interrogative} probings as indicators to estimate the model's understanding capability.  We will begin with a few preliminaries on generative AI.

%While generation capability can be simply measured by the success rate for model's generation to meet task requirement, how to evaluate understanding capability is less obvious as we have no means to access model's internal representation and reasoning procedure. Drawing inspirations from the cognitive procedure of human, we propose selective and interrogative probings as indicators to estimate model's understanding capability. We will first start with some preliminaries of generative models. 
% To test our hypothesis, we empirically evaluate the extent to which the model demonstrates an understanding capability alongside its impressive generative skills. The generation capability of a model is easily measurable by its success rate in fulfilling task requirements. However, assessing its understanding capability is less straightforward since we don't have means to access the model's internal representation and reasoning procedures. Taking inspiration from human cognitive processes, we propose using selective and interrogative probings as markers to estimate the understanding capability of the model. We will begin with a few preliminaries on generative models.
\subsubsection{Preliminaries of Generative AI}

\faeze{I think we can skip this preliminaries as we dicuss these details in the exp section. wdut?} \ximing{alternatively we can skip all the details in experiment? I feel it might be helpful to give an overview early in the paper, especially for saying people in NLP who's not familiar with how vision works.}
In language domain, it is the common practice is to have a unified language model $M$ (e.g. GPT-4) for all tasks and applications, which generates output text $\textbf{y}$ from an input text prompt $\textbf{x}$.

On the other hand, we have distinct models in vision domain. For image generation, we have a specialized generative model $M_G$ (e.g. DALL-E) which produces an image $\textbf{I}_y$ that corresponds to the input textual caption $\textbf{x}$. For general vision-language (VL) tasks such as visual question answering, we have a general-purpose VL model $M_D$ (e.g. BLIP-2) that outputs a text response $\textbf{y}$, in answer to the input text query $\textbf{x}$ based on the information from the input image $\textbf{I}_x$. Here, we consider discriminative VL models such as CLIP to be a special case of the general-purpose VL models which output a Boolean value $\textbf{y}$ to indicate if the input image $\textbf{I}_x$ corresponds to the input caption $\textbf{x}$.

%On the other hand, in vision domain, there are separate image generative model $M_G$ (e.g. DALL-E) and general-purpose vision-language model $M_D$ (e.g. BLIP-2, Bard) for image generation and solving vision-language tasks respectively. 

\subsubsection{Probe understanding as selection}
With a genuine understanding, it would be easier for humans to distinguish between correct and incorrect responses compared to generate the correct response \faeze{$\leftarrow$ I think by now we made this point clear. Also next sentence kind of say the same thing. how about removing the first sentence?} \ximing{sounds good}. Human often intuitively prefer multiple-choice questions and perform better on them compared to open-ended ones \cite{funkanddickson}. Inspired by this, we investigate whether a generative model, when capable of producing the correct answer in an open-ended format, can also consistently choose the correct option in a multiple-choice setting. Specifically, we assess the model's performance on identical tasks in both multiple-choice and open-ended formats, and then compare this to human performance in the same contexts. Formally, we denote the generative and discriminative accuracy of an agent as follows:
    \begin{align*}
    \small
        \text{Acc}_G(P_\theta) = \frac{\sum_{\textbf{x} \sim \mathcal{D}}\mathbbm{1}(\textbf{y} \in \hat{Y}), \textbf{y} \sim {P_\theta(\textbf{y}|\textbf{x})}}{\|\mathcal{D}\|}, \: \text{Acc}_D(P_\theta) = \frac{\sum_{(\textbf{x}, \hat{\textbf{y}}, C) \sim \mathcal{D}}\mathbbm{1}\big(\arg\max P_\theta(\textbf{y} | \textbf{x}, C) = \hat{\textbf{y}} \big)}{\|\mathcal{D}\|}
    \end{align*}
Here, $\theta$ represents an agent that can be either a model or a human. $\mathcal{D}$ denotes the test set for a specific task, $C$ denotes the set of candidates for a given query $\textbf{x}$. $\hat{\textbf{y}}$ is the ground-truth response, and $\hat{Y}$ represents the set of acceptable answers. In practice, we use human evaluation to determine if a generated response falls within the acceptable set.

For language, we use the unified model $M$ for both generation and selection. We explore a wide range of language-related tasks, such as dialogue, conversational QA, general QA, summarization, and commonsense reasoning. 
For tasks originally in multiple-choice format, like CSQA, we transformed them into generative tasks by omitting the candidates. 
Conversely, for tasks initially in a generative format, such as summarization, we changed them to multiple-choice by creating incorrect candidates.
We did this by perturbing the groundtruth response, for instance by introducing hallucinations. By adjusting the similarity between the incorrect and correct options, we can vary the difficulty of the multiple-choice task.

For vision, we use the generative model $M_G$ for image generation, and the general-purpose vision model $M_D$ for selection. Superficially, we prompt $M_G$ to generate images given the text descriptions, and ask $M_D$ to select the image, that better matches the text description from candidates.

\subsubsection{Probe understanding as interrogation}
With genuine understanding, a human would be able to answer basic questions about their own generation. Indeed, in oral exams, it's common to ask a series of questions based on prior answers to gauge a student's grasp of the subject. Similarly, we assess if a model can demonstrate a meaningful understanding of its own outputs by posing questions based on its own generated content. Concretely, we evaluate the model's question-answering performance given its own generated content as context. Formally,
    \begin{align*}
    \small
        \text{Acc}_U(P_\theta) = \frac{\sum_{\textbf{x} \sim \mathcal{D}}\mathbbm{1}(\textbf{r} \in \hat{R}), \textbf{r} \sim {P_\theta(\textbf{r}|\textbf{y})}, \textbf{y} \sim {P_\theta(\textbf{y}|\textbf{x})}}{\|\mathcal{D}\|}
    \end{align*}
For language, we first ask models to generate a paragraph-level text while taking into account some background information. We then ask model to use its generated content to answer background-related questions. For vision, we first prompt $M_G$ to generate images given the text descriptions, and then ask $M_D$ to answer questions about the content of these generated images.



%3 points we discussed:
%Discuss understanding and discrimination. 
%Notes from Yejin:
%ection 2: Overview table + list of observations

%\begin{enumerate}
%\item start by comparing humans vs AI in the intro: put forward the generative AI paradox which means Bla
%\item Intro: humans are worse than machines in generating impressive text. 
%\item the current situation raises the generative AI paradox:
%\item in this paper, provide news insights and reasons as to why these are the case: distractors and nature of the tasks, IID vs OOD 
%\item the goal is to shed light on the difference between AI intelligence and human intelligence. 
%\item compare LLMs in discrimination setup vs generation setup
%\item there are several dimensions for understanding 
%\item Compare human performance in discrimination and generation vs humans
%\item D
%\item organize different cases: what it means to understand:
%\item Different cells 

%A few more notes from Yejin:
%\begin{enumerate}
%    \item result is not binary
%    \item "in this paper we aim to answer this question by developing different formulation of the problem"
%    \item "curvature of intelligence in AI is more convoluted than expected"
%    \item "their curvature is highly fluctuating"
%    \item what people should cite us for: (1) "AI is not black magic in all dimensions" (2) generative AI and its limitations
%    \item use very low-key, plain language
%    \item make it more about asking questions
%    \item tone down the argument and it will have impact
%\end{enumerate}

%\item 


%\end{enumerate}

% Peter's comments:
% \begin{enumerate}
%     \item I really agree with how we framed what models are doing, although we will probably need to be careful about exactly how we state this in the paper. e.g. I do think comparative reasoning highlights why they fail, although there probably aren’t any universal breaks (like the elimination example) so we may need to be somewhat subtle/vague if and when we state this idea in the paper
% \item Likewise, really agree with thoughts about humans, but I’m guessing we’ll need to be fairly subtle/rely on reader commonsense for some of this, as there is still quite a bit of disagreement ito how humans learn and reason, and we don’t want to get caught in that debate
% \item I don’t think either above point means we should do things differently, just that we’ll need to be careful, and plan to do followup work where we might make stronger statements e.g. to do a more comprehensive empirical study of why the paradox happens, where I’m guessing we’ll need to spend more space in this paper simply proving that it happens at all
% \end{enumerate}

$ $

%breif operationized definition
%see appendix for comprehensive literature





==> sections/history/2_hypotheses_v2.tex <==
\section{The Generative AI Paradox}

\peter{Temporary draft, to help us plan for experiments etc. Feel free to comment, although some of this may be overwritten with a new version later today (Tuesday)}

\subsection{Operational Definitions}

Figure~\ref{fig:gen-example} offers an example of the seemingly paradoxical behavior of generative models. In language (centre-left), GPT-4 is able to generate a compelling story about 3 friends building a house, but when pressed on details of its \emph{own generated story}, fails to correctly answer a simple question: GPT-4 claims only one design was sketched for the house despite writing that they spent years ``sketching designs''. In vision (centre-right), a generator produces a correct image beyond average human capabilities, yet the understanding model is unable to single out that correct generation against plausible alternatives, despite this selection being the seemingly ``easier'' task. In both cases, models seem to meet or exceed human generation abilities but lag in understanding. \peter{This may change if we change the motivating examples}

\peter{Fix this beginning} Observations such as these motivate the Generative AI Paradox:

\begin{displayquote}

\emph{Generative models seem to acquire generation abilities more easily than understanding, which stands in contrast to human intelligence where generation is usually harder and may require understanding.}

\end{displayquote}

\peter{optional math: (can easily drop this, just use the text)} 
To test this requires an operational definition of each aspect of the paradox. First, what it means for generation to be ``easier'' than understanding, taking human intelligence as a baseline. We more formally define this paradox as: 


\begin{equation} 
\begin{split} \label{eq:paradox}
&\exists T_{p} \subset T,\ |T_{p}|>k\ \ s.t.\ \ \forall t \in T_{p}  \\
&\textbf{g}(human,t) = \textbf{g}(model,t) \implies \textbf{u}(human, t) - \textbf{u}(model, t) >  \epsilon 
\end{split}
\end{equation}

Put simply, there is a subset of tasks $T_{p}$ of a reasonable size ($>k$) where a human who achieves the same generation performance $\textbf{g}$ as a model would be expected to achieve significantly ($>\epsilon$) higher understanding performance $\textbf{u}$ than the model did. Stated another way, models underperform human expectation in understanding, given their strong generation capabilities.

Generation performance $\textbf{g}$ has a straightforward operational definition, as it is based on the observable behavior of producing content which can then be evaluated automatically or by humans. 
Understanding is not a directly operational concept, but measuring understanding performance $\textbf{u}$ is frequently done when evaluating humans. We consider 2 common methods:
\begin{enumerate}
    \item \textbf{Selective evaluation} in which understanding is demonstrated by selecting a correct option for a given query. A common example of this is multiple choice question answering, which is one of the most common ways to examine human understanding (CITE), as well as natural language understanding in language models (CITE). This corresponds to (X) in Figure~\ref{fig:gen-example}.
    \item \textbf{Interrogative evaluation} in which understanding is tested with a series of probing questions to draw out the overall understanding of content. A common example of this is oral examination in education (CITE). This corresponds to (X) in Figure ~\ref{fig:gen-example}
\end{enumerate}

Together with Hypothesis~\ref{eq:paradox}, these provide us with a blueprint for evaluating the Generative AI Paradox, by testing whether this holds for definitions of understanding across modalities and tasks.

\subsection{Experimental Overview}

Here, we provide a high-level road map for experiments informed by the definitions above.

\subsubsection{Hypotheses}

Evaluating whether Hypothesis~\ref{eq:paradox} holds for a given task requires establishing a human baseline, specifically, the understanding performance we expect from a human with the same generative capabilities as the model. 

\paragraph{selective evaluation} In this setting (i.e. multiple choice) common wisdom tells us that humans tend to have an easier time discriminating between reasonable options for a given task prompt, than generating a new one (CITE). Thus, we look here for cases where models lag in selective understanding given equal or even worse generation by humans. \lindsey{the selection in vision is still on generated images, though we have results on real images as well. I believe some of the hard negatives in language are also generated.} The sub-hypothesis in these cases is:

\underline{sub-hypothesis 1:} \emph{models exceed humans at generation while lagging at discrimination}. 

\paragraph{interrogative evaluation} We make the logical assumption that humans \emph{tend to be able to answer simple questions of understanding about their own generations.} For a given task input, we then test model accuracy for understanding questions, implicitly assuming that humans would get near perfect on such questions for their own generations, and taking this as the human baseline. The sub-hypothesis in this case would be:

\underline{sub-hypothesis 2:} \emph{models struggle to answer simple questions about generated content, which humans could answer for their own generations}. 

\subsubsection{Modalities and Models}
We focus our study on the strongest current generative models, particularly those that are driving interest and concern among experts and the public. We thus investigate the modalities of language and vision, where the most recent and impressive progress has been made. Within language, we use GPT-4 and ChatGPT as both generation and understanding models. In the vision domain, the strongest generators and understanding models are typically separate. We use Midjourney (CITE) as our generating model, CLIP~\cite{} and OpenCLIP~\cite{} as our understanding models for selective evaluation, and BLIP-2~\cite{}, BingChat~\cite{} and Bard~\cite{} for interrogative evaluation.  \lindsey{maybe too many models on vision part? and will add the citations.}


\subsubsection{Experiments}

We break our study into 2 sections: \S\ref{} for sub-hypothesis 1: selective understanding (\S\ref{} for language and \S\ref{} for vision) and \S\ref{} for sub-hypothesis 2: interrogative understanding (\S\ref{} for language and \S\ref{} for vision).


% \subsection{(Leftover from previous \S2)}

% \subsection{Representative Models and Tasks for Language and Vision}
% \nouha{work in progress, don't look yet. I'm updating text, tables and adding new plots} 
% We explore the paradox from different angles across different tasks within two distinct modalities: language and vision.
% We conduct two categories of experiment in these modalities: 1) analysis of models generative vs discriminative abilities for a given task/prompt, and 2) analysis of models' ability to answer questions about their own generations [this sentence can be moved before introducing the models which I think is what you do in Sec2].


% % For each task, we consider two settings for evaluation: \textbf{i) generative:} we prompt models to generate a response given task-specific inputs (e.g., dialogue history, document, premise, image caption etc.), and \textbf{ii) discriminative:} we require the models to select the correct answer from a set of candidates.

% % \ake{We conduct two categories of experiment in these modalities: 1) analysis of models generative vs discriminative abilities for a given task/prompt, and 2) analysis of models' ability to answer questions about their own generations.}


% \subsubsection{Language Models and Tasks}


% % LMs exhibit remarkable proficiency in generating content. They can craft intricate stories, generate visually stunning artworks, or even compose music that can be indistinguishable from human creations. However, where these models tend to lag behind is in their ability to discriminate effectively. We consider a wide variety of tasks. \faeze{later add a table with all tasks stat and refer here} from the language and vision modality to show this paradox. 


% %\input{figures/generation_example}
% % \subsection{Experimental Setup}

% % \ake{First we compare generation vs discrimination capabilities in both language and vision models.... }

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/language/main_fig_disc_gen_gpt4_human-cropped.pdf}
% %     \caption{GPT4 generative and discriminative performance versus human performance. While models exhibit strong capabilities in generating answers, they lag in discriminating between a set of answers when compared to human performance. The same trend applies for ChatGPT (See Appendix \S\ref{fig:chatgpt_exp1_language}.}
% %     \vspace{-15pt}
% %     \label{fig:expt1-main-results}
% % \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/language/exp1_disc_vs_gen_v2.pdf}
%     \caption{ChatGPT, GPT4 and human performances under the generative and discriminative task formulation. See Appendix \S\ref{fig:chatgpt_exp1_language} for ChatGPT performance on all the tasks. \faeze{sure, we will decide at the end. I will make the other version too. btw I can also remove gridlines if that will help} \liwei{this seems to be too small to read?} \faeze{Liwei, do you mean the bar values? I can increase them}}
%     \label{fig:expt1-main-results-v2}
% \end{figure}

% \noindent{\textbf{Models.}} To understand the capabilities of LLMs, we evaluate \textbf{ChatGPT} (\texttt{GPT-3.5-turbo}) \cite{team2022chatgpt} and \textbf{GPT4} (\texttt{gpt-4}) \cite{openai2023gpt4}  using zero-shot prompting. We examine a diverse array of language-related tasks, including dialogue, conversational QA, general QA, summarization, and commonsense reasoning. These tasks span a spectrum from open-ended, where the model enjoys greater freedom to generate output, to more tightly constrained tasks, where the model must adhere to specific guidelines while generating responses.

% \noindent{\textbf{Benchmarks}.} In the dialogue domain, we explore both open-ended datasets namely \textbf{Mutual}$^+$  \cite{cui-etal-2020-mutual} and \textbf{DREAM} \cite{sun-etal-2019-dream}, as well as a document-grounded benchmark, \textbf{Faithdial} \cite{dziri2022faithdial}. These tasks involve generating coherent continuations based on the conversation history while also being faithful to the document (in the case of grounded dialogue). For reading comprehension, we experiment on \textbf{Topioca} \cite{adlakha2022topiocqa}, a conversational QA dataset. We also consider a factual QA dataset  \textbf{RACE} \cite{lai-etal-2017-race}. % and  \textbf{Vitamin 
% For summarization, we consider \textbf{XSUM} \cite{narayan-etal-2018-dont}. For commonsense reasoning, we experiment on a series of benchmarks:  \textbf{CommonSenseQA} \cite{talmor-etal-2019-commonsenseqa}, \textbf{SocialIQA} \cite{sap-etal-2019-social}, \textbf{HellaSwag} \cite{zellers-etal-2019-hellaswag}, \textbf{PIQA} \cite{seo2018phrase}, \textbf{$\alpha$NLG/$\alpha$NLI} \cite{bhagavatula2020abductive} and lastly we considered NLI tasks including \textbf{WaNLI} \cite{liu-etal-2022-wanli}, and \textbf{$\delta$-NLI} \cite{rudinger-etal-2020-thinking}.



% \subsubsection{Vision Models and Tasks}

% % \paragraph{Vision Models and Benchmarks.} 
% \noindent{\textbf{Models.}}
% Unlike the language domain, where generation and understanding have been unified into one model, different models are used in practice for image generation and understanding. Thereby, we broadly divide vision models into two categories, based on their use cases: \textbf{$i$) image generation models}~\cite{ramesh2021zero,stablediffusion,yu2022scaling}, \lindsey{we can cite these related works in intro or section 2 when image generation model first appears. feel these are too much for experiment section.} which can generate images given a text prompt. In our study, we specifically consider \textbf{Midjourney}\footnote{\url{https://www.midjourney.com}} as our image generator model. And, \textbf{$ii$) image understanding models}, 
% which can answer questions about an image~\cite{li2022blip,wang2022git,driess2023palm,openai2023gpt4}, or 
% measure the similarity between a text description and the input image. For this study, we leverage both \textbf{CLIP} \cite{radford2021learning} and \textbf{OpenCLIP} \cite{ilharco_gabriel_2021_5143773} models, that are widely adopted for image-text similarity measure.  \lindsey{will add the models for interrogative evaluation here.}

% \noindent{\textbf{Benchmarks}.} To evaluate model's capability of image generation, we consider 4 benchmarks to source text prompts. These text prompts span from descriptions about natural scenes, which are most likely to be in-domain for the model to generate, to out-of-distribution scenes which challenge the model to generate objects with specific attributes and relationships that rarely exist in real images. Specifically, the text prompts are sourced from the following datasets: \textbf{COCO}~\cite{lin2014microsoft}, \textbf{PaintSkill}~\cite{Cho2022DallEval}, \textbf{DrawBench}~\cite{saharia2022photorealistic} and \textbf{T2ICompBench}~\cite{huang2023t2icompbench}. \lindsey{and also add the TIFA v.10 dataset here.}
% \footnote{ COCO prompts are human-written captions on real images. PaintSkill features text prompts that examine image generation on specific object categories, object counts and spatial relations between objects. DrawBench additionally test for long-form text, rare words, and challenging prompts. T2ICompBench is designed to test models on open-world, compositional text-to-image generation, with text prompts covering 3 categories, attribute binding, object relationships, and complex compositions. In practice, we randomly sample 100 text prompts from each dataset. \nouha{Maybe we can even move these details to Appendix} \lindsey{yes, let's move to appendix.}}. We use the same text prompts, with pairs of generated images for discriminative evaluation. Refer to \S\ref{} for more details about the datasets.

% % \nouha{For image discrimination/understanding, we use prompts and images from the same datasets, no? if yes, we can edit the text to reflect that} \lindsey{will add a sentence at the end mentioning that.}

% % \lindsey{I removed tifa from exp4.1, cuz we are mostly using it for exp4.2. and tifa is actually a composition of the 4 datasets above. May consider to move the description about each dataset to appendix, if we are over space limit.} \nouha{Yes!!}

% % \lindsey{a general question, are we only talking about the setup of exp 1 and exp4.1 here?}

% % \nouha{Here's we talking about exp1, how discrimination lags compared to generation} \lindsey{got it.}

% % \nouha{hey Lindsey, I'm thinking we can have the same figures as language for vision for exp1. We don't have human generation accuracy but that's fine. We can assume that humans on average will do poorly compared to models in producing images, but we can have the discrimination vs generation plot fot different models and we can compare against human discrimination no?}

% % \lindsey{I am assuming this is Figure 3? We can probably just put close to 0 for human generative. Do you have suggestions on which model we put for discriminative? maybe just the one that got the best performance? i.e., open-clip: CLIP-ViT-bigG-14-laion2B-39B-b160k} 
% % \nouha{TBH, it's dangerous to put 0 as expert painters can be excellent at drawing but significantly slower. I picked the best models and added them to the same vision sheet, "plots" tab. You can add things there.}

% % \nouha{Let's not plot 0 as human generative performance but rather mention it in text.}

% % \lindsey{another question on how to present vision results, figure 3 was on discriminative NLP tasks? we do not have an exact equivalent on vision. We probably can just use hard negative setting results for vision figure 3, as that is the actual user case when use image generation models. One concern is the same results will be repeated for figure 4.}

% % \nouha{For the ablation hard/easy for discrimination, we can add a vision plot to Fig 4}

% % \lindsey{yes, will add a vision plot similar to Fig 4.}









==> sections/history/2_hypotheses_v3.tex <==
\section{The Generative AI Paradox}

We begin by outlining the Generative AI Paradox, and experimental design to test it.

\subsection{Operational Definitions}

Figure~\ref{fig:gen-example} offers an example of the seemingly paradoxical behavior of generative models. In language (centre-left), GPT-4 is able to generate a compelling story about 3 friends building a house, but when pressed on details of its \emph{own generated story}, fails to correctly answer a simple question: GPT-4 asserts that only one design was sketched in the story despite writing that they spent years ``sketching designs''. In vision (centre-right), a generator produces a correct image beyond average human capabilities, yet the understanding model is unable to single out that correct generation against plausible alternatives, despite this selection being the seemingly ``easier'' task. In both cases, models meet or exceed human generation abilities but lag in understanding. \peter{This may change if we change the motivating examples}

Observations such as these motivate the Generative AI Paradox:

\begin{displayquote}

\emph{Generative models seem to acquire generation abilities more easily than understanding, which stands in contrast to human intelligence where generation is usually harder or requires understanding.}

\end{displayquote}

\peter{optional math: (can easily drop this, replace with equivalent text)} \yejin{oh this is so cute; let's keep it} \jillian{I rewrote the math section to be more similar to stats papers but kept the original in comment below, feel free to change it back. } \peter{Will review all of section 2 soon, and may take a combination of the 2 that balances the different aspects}
To test this requires an operational definition of each aspect of the paradox. First, what it means for generation performance $\textbf{g}(entity, task)$  to be ``easier'' than understanding performance $\textbf{u}(entity, task)$, taking human intelligence as a baseline. We consider a subset of tasks $T_{p} \subset T $ from all tasks $T$, where $|T_{p}|>k$. Using this notation, we formally define this paradox for all $t \in T_{p}$ as: 

\begin{equation} 
\label{eq:paradox}
\textbf{g}(human,t) = \textbf{g}(model,t) \implies \textbf{u}(human, t) - \textbf{u}(model, t) >  \epsilon 
\end{equation}

Put simply, there is a subset of tasks $T_{p}$ of a reasonable size ($>k$) where a human achieves the same generation performance $\textbf{g}$ as a model but, in contrast,  achieves significantly ($\epsilon>0$) higher understanding performance $\textbf{u}$ than the model. \ake{something that came out as I was going through the results section is that ``generation performance'' has at least two dimensions---stylistic quality and accuracy of content---and that distinction probably matters a lot when comparing to humans, who may not be able to match the style but probably won't suffer on generation accuracy} Stated another way, models underperform human expectation in understanding, given their strong generation capabilities.

% To test this requires an operational definition of each aspect of the paradox. First, what it means for generation to be ``easier'' than understanding, taking human intelligence as a baseline. We more formally define this paradox as: 


% \begin{equation} 
% \begin{split} \label{eq:paradox}
% &\exists T_{p} \subset T,\ |T_{p}|>k\ \ s.t.\ \ \forall t \in T_{p}  \\
% &\textbf{g}(human,t) = \textbf{g}(model,t) \implies \textbf{u}(human, t) - \textbf{u}(model, t) >  \epsilon 
% \end{split}
% \end{equation}

% Put simply, there is a subset of tasks $T_{p}$ of a reasonable size ($>k$) where a human who achieves the same generation performance $\textbf{g}$ as a model would be expected to achieve significantly ($>\epsilon$) higher understanding performance $\textbf{u}$ than the model did. Stated another way, models underperform human expectation in understanding, given their strong generation capabilities.

Generation performance $\textbf{g}$ has a straightforward operational definition, as it is based on the observable behavior of producing content which can then be evaluated automatically or by humans. 
Understanding is not a directly operational concept, but measuring understanding performance $\textbf{u}$ is frequently done when evaluating humans. We consider 2 common methods \ake{this seems like a reasonable formulation/description of the two types---we should decide on one and then make consistent across intro, this section, and experimental sections. one note is that this characterization focuses on the format of the questions, rather than the content}:
\begin{enumerate}
    \item \textbf{Selective evaluation} in which understanding is demonstrated by selecting a correct option for a given query or prompt. A common example of this is multiple choice question answering, which is one of the most common ways to examine human understanding (CITE), as well as natural language understanding in language models (CITE). This corresponds to (X) in Figure~\ref{fig:gen-example}. 
    \item \textbf{Interrogative evaluation} in which understanding is tested with a series of probing questions to draw out the overall understanding of content. A common example of this is oral examination in education (CITE). This corresponds to (X) in Figure ~\ref{fig:gen-example}
\end{enumerate}

This provide us with a blueprint for evaluating the Generative AI Paradox, by testing whether Hypothesis~\ref{eq:paradox}, holds for definitions of understanding across modalities, tasks, and models. 

\subsection{Experimental Overview}

Here, we provide a high-level road map for experiments informed by the definitions above. We propose 2 sub-hypotheses to test across experimental settings, and provide cross-experiment details.

\subsubsection{Hypotheses}

\peter{This section could be clearer/more concise}
Evaluating whether Hypothesis~\ref{eq:paradox} holds for a given task requires establishing a human baseline, specifically, the understanding performance we expect from a human with the same generative capabilities as the model. 

\paragraph{selective evaluation} In this setting (i.e. multiple choice) common wisdom tells us that humans tend to have an easier time discriminating between reasonable options for a given task prompt, than generating a new one (CITE) \ake{I'm not sure it's actually as necessary to establish that this is difficult/easy for humans---rather it seems more important to justify why this is a good test of understanding, and then you could predict that models will underperform humans}. Thus, we look here for cases where models lag in selective understanding given equal or even worse generation by humans. \lindsey{the selection in vision is still on generated images, though we have results on real images as well. I believe some of the hard negatives in language are also generated.} The sub-hypothesis in these cases is:

\underline{sub-hypothesis 1:} \emph{models exceed humans at generation while lagging at discrimination}. 

\paragraph{interrogative evaluation} We make the logical assumption that humans \ake{similarly here, might be good to frame in terms of how this is a test of understanding} \emph{tend to be able to answer simple questions of understanding about their own generations.} For a given task input, we test model accuracy for understanding questions on AI generated outputs and as the human baseline, assume that humans would get near perfect accuracy on such questions for their own generations. The sub-hypothesis in this case would be:

\underline{sub-hypothesis 2:} \emph{models struggle to answer simple questions about generated content, which humans could answer for their own generations}. 

\subsubsection{Modalities and Models}
We focus our study on the strongest current generative models, particularly those that are driving interest and concern among experts and the public. We thus investigate the modalities of language and vision, where the most recent and impressive progress has been made. Within language, we use GPT-4 and ChatGPT as both generation and understanding models. In the vision domain, the strongest generators and understanding models are typically separate. We use Midjourney\footnote{\url{https://midjourney.com}} as our generating model, CLIP~\cite{radford2021learning} and OpenCLIP~\cite{ilharco_gabriel_2021_5143773} as our understanding models for selective evaluation, and BLIP-2~\cite{li2023blip}, BingChat\footnote{\url{https://bing.com/chat}} and Bard\footnote{\url{https://bard.google.com}} for interrogative evaluation. \lindsey{added the citation, for Midjourney, BingChat, Bard, added the url. lmk if there is a more proper way to cite a website for ICLR.}
 % \lindsey{maybe too many models on vision part? and will add the citations.}


\subsubsection{Experiments}

We break our study into 2 sections below: \S\ref{} for sub-hypothesis 1: selective understanding (\S\ref{} for language and \S\ref{} for vision) and \S\ref{} for sub-hypothesis 2: interrogative understanding (\S\ref{} for language and \S\ref{} for vision).



==> sections/history/2_hypothesis_v4.tex <==
\section{The Generative AI Paradox}

\peter{!!! WILL DROP A NEW VERSION IN SOON}

We begin by outlining the Generative AI Paradox, and experimental design to test it.

\subsection{Operational Definitions}

\peter{This paragraph will change once Figure~\ref{fig:gen-example} converges} Figure~\ref{fig:gen-example} offers an example of the seemingly paradoxical behavior of generative models. In language (centre-left), GPT-4 is able to generate a compelling story about 3 friends building a house, but when pressed on details of its \emph{own generated story}, fails to correctly answer a simple question: GPT-4 asserts that only one design was sketched in the story despite writing that they spent years ``sketching designs''. In vision (centre-right), a generator produces a correct image beyond average human capabilities, yet the understanding model is unable to single out that correct generation against plausible alternatives, despite this selection being the seemingly ``easier'' task. In both cases, models meet or exceed human generation abilities but lag in understanding. 

Observations such as these motivate the Generative AI Paradox:

\begin{displayquote}

\emph{Generative models seem to acquire generation abilities more easily than understanding, which stands in contrast to human intelligence where generation is usually harder or requires understanding.}

\end{displayquote}

%\peter{optional math: (can easily drop this, replace with equivalent text)} \yejin{oh this is so cute; let's keep it} \jillian{I rewrote the math section to be more similar to stats papers but kept the original in comment below, feel free to change it back. } \peter{Will review all of section 2 soon, and may take a combination of the 2 that balances the different aspects}
To test this requires an operational definition of each aspect of the paradox. First, what it means for generation performance for a given model and task $\textbf{g}(model, task)$  to be ``easier'' than understanding performance $\textbf{u}(model, task)$, taking human intelligence as a baseline. We formally state the paradox \faeze{hypothesis?} as: 

\begin{equation} 
\label{eq:paradox}
\textbf{g}(human,t) = \textbf{g}(model,t) \implies \textbf{u}(human, t) - \textbf{u}(model, t) >  \epsilon 
\end{equation}

Put simply, there is a subset of tasks $T_{p}$ of a reasonable size ($>k$) where a human who achieves the same generation performance $\textbf{g}$ as a model would be expected to achieve significantly ($>\epsilon$) higher understanding performance $\textbf{u}$ than the model did. 
%\ake{something that came out as I was going through the results section is that ``generation performance'' has at least two dimensions---stylistic quality and accuracy of content---and that distinction probably matters a lot when comparing to humans, who may not be able to match the style but probably won't suffer on generation accuracy} \peter{Agree, although maybe we can kind of leave this vague here (``given some notion of generation performance...'') as the stylistic aspect may be more of a ``why'' than a ``what'' for ease/preference of machine generations? Open to changing it though!} 
Stated another way, models underperform human expectation in understanding, given their strong generation capabilities.

% To test this requires an operational definition of each aspect of the paradox. First, what it means for generation to be ``easier'' than understanding, taking human intelligence as a baseline. We more formally define this paradox as: 


% \begin{equation} 
% \begin{split} \label{eq:paradox}
% &\exists T_{p} \subset T,\ |T_{p}|>k\ \ s.t.\ \ \forall t \in T_{p}  \\
% &\textbf{g}(human,t) = \textbf{g}(model,t) \implies \textbf{u}(human, t) - \textbf{u}(model, t) >  \epsilon 
% \end{split}
% \end{equation}

% Put simply, there is a subset of tasks $T_{p}$ of a reasonable size ($>k$) where a human who achieves the same generation performance $\textbf{g}$ as a model would be expected to achieve significantly ($>\epsilon$) higher understanding performance $\textbf{u}$ than the model did. Stated another way, models underperform human expectation in understanding, given their strong generation capabilities.

Generation performance $\textbf{g}$ has a straightforward operational definition, as it is based on the observable behavior of \faeze{consider removing "as it is based on the observable behavior of" and add ---} producing content which can then be evaluated automatically or by humans. We particularly focus on notions of generation quality related to style, correctness, and human preference.
Understanding is not a directly operational concept, but measuring understanding performance $\textbf{u}$ is frequently done when evaluating humans. We consider 2 common methods \ake{this seems like a reasonable formulation/description of the two types---we should decide on one and then make consistent across intro, this section, and experimental sections. one note is that this characterization focuses on the format of the questions, rather than the content}: \peter{Just to clarify, would the content mean the \emph{kind} of questions that are asked?}
\begin{enumerate}
    \item \textbf{Selective evaluation} in which understanding is demonstrated by selecting a correct option for a given query or prompt. A common example of this is multiple choice question answering, which is one of the most common ways to examine human understanding (CITE), as well as natural language understanding in language models \citep{wang2018glue}. This corresponds to (a) columns in Figure~\ref{fig:gen-example}. 
    \item \textbf{Interrogative evaluation} in which understanding is tested with a series of probing questions to draw out the overall understanding of (generated) content. A common example of this is an oral examination in education (CITE). This corresponds to (b) columns in Figure ~\ref{fig:gen-example}
\end{enumerate}

\faeze{Do we want to talk about selective/interrogative both in 201 and 2.2? If we deicide to keep both maybe one should be very brief? } \peter{We'll probably push more to \S2.1, and focus on giving intuition for the actual experiments in \S2.2. Working on this now. Agree that length could be less}
This provides us with a blueprint for evaluating the Generative AI Paradox, by testing whether Hypothesis~\ref{eq:paradox}, holds for definitions of understanding across modalities, tasks, and models. 

\subsection{Experimental Overview}

Here, we provide a high-level road map for experiments informed by the definitions above. We propose 2 sub-hypotheses to test across experimental settings, and provide cross-experiment details.

\subsubsection{Hypotheses}

\peter{This section could be clearer/more concise}

Evaluating whether Hypothesis~\ref{eq:paradox} holds for a given task requires establishing a human baseline, specifically, the understanding performance we expect from a human with the same generative capabilities as the model. 

\paragraph{selective evaluation} In this setting (i.e. multiple choice) common wisdom tells us that humans tend to have an easier time discriminating between reasonable options for a given task prompt, than generating a new one (CITE) \ake{I'm not sure it's actually as necessary to establish that this is difficult/easy for humans---rather it seems more important to justify why this is a good test of understanding, and then you could predict that models will underperform humans} \peter{Wondering if establishing this will fit better in the previous section? As this is where we introduce selective/interrogative eval as valid ways of measuring understanding. The original intention of hypotheses section was to establish exactly what result we're looking for and why this would like up with Hypothesis~\ref{eq:paradox}. Will revise!}. Thus, we look here for cases where models lag in selective understanding given equal or even worse generation by humans. \lindsey{the selection in vision is still on generated images, though we have results on real images as well. I believe some of the hard negatives in language are also generated.} The sub-hypothesis in these cases is:

\underline{sub-hypothesis 1:} \emph{models exceed humans at generation while lagging at discrimination}. 

\paragraph{interrogative evaluation} We make the logical assumption that humans \ake{similarly here, might be good to frame in terms of how this is a test of understanding} \emph{tend to be able to answer simple questions of understanding about their own generations.} For a given task input, we test model accuracy for understanding questions on AI generated outputs and as the human baseline, assume that humans would get near perfect accuracy on such questions for their own generations. The sub-hypothesis in this case would be:

\underline{sub-hypothesis 2:} \emph{models struggle to answer simple questions about generated content, which humans could answer for their own generations}. 

\subsubsection{Modalities and Models}
We focus our study on the strongest current generative models, particularly those that are driving interest and concern among experts and the public. We thus investigate the modalities of language and vision, where the most recent and impressive progress has been made. Within language, we use GPT-4 and ChatGPT as both generation and understanding models. In the vision domain, the strongest generators and understanding models are typically separate. We use Midjourney\footnote{\url{https://midjourney.com}} as our generating model, CLIP~\cite{radford2021learning} and OpenCLIP~\cite{ilharco_gabriel_2021_5143773} as our understanding models for selective evaluation, and BLIP-2~\cite{li2023blip}, BingChat\footnote{\url{https://bing.com/chat}} and Bard\footnote{\url{https://bard.google.com}} for interrogative evaluation. 
%\lindsey{added the citation, for Midjourney, BingChat, Bard, added the url. lmk if there is a more proper way to cite a website for ICLR.}
 % \lindsey{maybe too many models on vision part? and will add the citations.}


\subsubsection{Experiments}
\pw{probably don't need a separate subsubsection just to say this? you can put it at the start of the next section} \peter{the issue is that this covers 2 sections (3 + 4) so having it at the beginning of \S\ref{sec:exp1} would be unbalanced. We might rearrange this section a bit so that this makes more sense though}
We break our study into 2 sections below: \S\ref{sec:exp1} for sub-hypothesis 1: selective understanding (\S\ref{} for language and \S\ref{} for vision) and \S\ref{sec:exp2} for sub-hypothesis 2: interrogative understanding (\S\ref{} for language and \S\ref{} for vision).



==> sections/history/3_experiments_v1.tex <==
\section{Experiments}
\nouha{work in progress}

\subsection{Experimental Setup}
\paragraph{Language} To understand the capabilities of LLMs, we evaluateChatGPT (\texttt{GPT-3.5-turbo}) \cite{team2022chatgpt} and GPT4 (\texttt{gpt-4}) \cite{openai2023gpt4}  using zero-shot prompting.

\paragraph{Vision}

\subsection{Models excel at generation while lagging at Discrimination}

\nouha{work in progress, don't look yet. I'm updating text, tables and adding new plots}

LMs exhibit remarkable proficiency in generating content. They can craft intricate stories, generate visually stunning artworks, or even compose music that can be indistinguishable from human creations. \nouha{This can go to intro}. However, where these models tend to lag behind is in their ability to discriminate effectively. Discrimination refers to the capacity to make accurate and nuanced distinctions between different inputs.  We consider a wide variety of tasks \faeze{later add a table with all tasks stat and refer here} from the language and vision modality to show this paradox. 



\paragraph{Language Tasks}
We examine a diverse array of language-related tasks, including dialogue, conversational QA, general QA, summarization, and commonsense reasoning. These tasks span a spectrum from open-ended, where the model enjoys greater freedom to generate output, to more tightly constrained tasks, where the model must adhere to specific guidelines while generating responses.

In the domain of open-ended dialogue, we explore two datasets: \textbf{Mutual}$^+$  \cite{cui-etal-2020-mutual} and \textbf{DREAM} \cite{sun-etal-2019-dream}. These tasks involve generating coherent continuations based on the conversation history. For reading comprehension, we use \textbf{Topioca} \cite{adlakha2022topiocqa}, a conversational question-answering dataset. We also consider factual QA datasets such as  \textbf{RACE} \cite{lai-etal-2017-race}, as well as two counterfactual QA benchmarks, namely  \textbf{ARC}  \cite{} and  \textbf{Vitamin C} \cite{schuster-etal-2021-get}.
Additionally, we considered \textbf{Faithdial} \cite{dziri2022faithdial}, a document-grounded dialogue benchmark where the task is to both generate a faithful response aligned with the document and a response that maintains coherence with the conversation history. We also examine \textbf{XSUM} \cite{narayan-etal-2018-dont} for summarization.   For commonsense reasoning, we considered a series of benchmarks:  \textbf{CommonSenseQA} \cite{talmor-etal-2019-commonsenseqa}, \textbf{SocialIQA} \cite{sap-etal-2019-social}, \textbf{HellaSwag} \cite{zellers-etal-2019-hellaswag}, \textbf{PIQA} \cite{seo2018phrase}, and lastly we considered NLI tasks including \textbf{WaNLI} \cite{liu-etal-2022-wanli} and \textbf{delta-NLI} \cite{rudinger-etal-2020-thinking}.


\paragraph{Vision Tasks}




\paragraph{Setup} For each task, we consider two settings: \textbf{i) generative:} we prompt GPT4 and ChatGPT to generate a response given provided background information (e.g., dialogue history, document, premise, etc). \textbf{ii) discriminative:} we require the models to select the correct answer from a set of candidates.  

\paragraph{Ablation Study on the discriminative setup}
For tasks originally designed to be generative, we constructed a candidate set $N$ comprising $N-1$ negative candidates and the groundtruth answer.  To generate the negative answers, we considered 3 approaches: \textbf{1) hard negatives}:  These are particularly challenging examples designed to make it difficult for models to rely on data biases and artifacts to produce an answer. They contain subtle incorrect information that challenges the models' ability to recognize the errors unless they possess a profound understanding of the task. \textbf{2) moderately hard negatives}: These candidates are semantically close to the groundtruth answer, but their errors are more noticeable for the models.
and \textbf{3) easy negatives}: These candidates are semantically distant from the topic of the question, providing a clear contrast to the correct answer. 
To evaluate the quality of responses for the generative setting, we hire workers from Amazon Mechanical Turk (AMT) (See details in Appendix \S\ref{}). In the discriminative setting, we measure the accuracy of the models choosing the groundtruth answer.

\paragraph{Results} Results are shown in Table~\ref{tab:my_label} \nouha{this is temporary}. Our findings depict a multifaceted landscape, characterized by the model's behavior exhibiting significant variability across various tasks and configurations. Notably, in numerous language-related tasks, we observe a preference for model-generated content over human-generated content, despite the models potentially lagging behind humans in their ability to genuinely understand and select the correct answers.




% \begin{table}[t!]
%     \centering
%   \footnotesize
%     \input{tables/exp1_results}
%      \caption{Caption: \nouha{reporting the hard negative for the discriminative accuracy, will add another table to show the difference between hard and easy. Hard and easy are not applicable for all the tasks, this is why I moved it to a new table.} \faeze{I think having a pot similar to figure \ref{fig:disc_colllie} with their generative vs discriminative performance next to each other is nice and makes the comparison easier. I can do that if you agree on having plots  } \nouha{Good idea, was thinking of that as well. Just having this table now to get a sense of what we have vs not. For each dataset, we can have 1) GPT4/ChatGPT generative vs Human generative (working on running this) and 2) GPT4/ChatGPT discriminative vs Human discriminative) I will add the plots once the experiment is done.}}
%     \label{tab:my_label}
% \end{table}


%%% Consensing the table


\begin{table}[t!]
    \centering
  \footnotesize
   
\begin{tabular}{ |p{2cm}||p{1.5cm}|p{2cm}| p{2cm} | p{2cm} | p{2cm} |}
 \hline
Domain & Dataset & Model  & Generative quality (H) & Discriminative Accuracy (M) & Human Discri Accuracy\\
\hline
\multirow{8}{*}{Dialogue} & \multirow{2}{*}{FaithDial}  & {GPT4}  & {0.83} & {0.63} & \multirow{2}{*}{0.86}\\
 & & {ChatGPT} & 0.89 & 0.60 & \\
\cline{2-6}
& \multirow{2}{*}{DREAM} & GPT4  & 0.96 & 0.96 & \multirow{2}{*}{0.96}\\
 & & ChatGPT  & 0.97 & 0.90 & \\
\cline{2-6}
& \multirow{2}{*}{Mutual$^+$} & GPT4  & 0.99 & 0.76 & \multirow{2}{*}{0.80}\\
 & & ChatGPT  & 0.99 & 0.63 & \\
\hline
\multirow{2}{*}{Conv. QA} & \multirow{2}{*}{Topioca}  &{GPT4}  & 0.93 & 0.92 & \multirow{2}{*}{0.92}\\
 & & {ChatGPT}  & 0.92 & 0.88 & \\
\hline
\multirow{4}{*}{QA} & \multirow{2}{*}{RACE} & GPT4  & 0.96 & 0.89 & \multirow{2}{*}{0.82}\\
 & & ChatGPT  & 0.94 & 0.83 & \\
\cline{2-6}
& \multirow{2}{*}{ARC}  & GPT4  & 0.95 & 0.95 &  \multirow{2}{*}{x}\\
 & & ChatGPT & 0.96 & 0.82 & \\
\hline
\multirow{2}{*}{Summarization} & \multirow{2}{*}{XSUM} & {GPT4}  & 0.99 & 0.19 & \multirow{2}{*}{0.84}\\
& & ChatGPT & 0.99  & 0.10 &\\

\hline
\multirow{10}{*}{Commonsense} & \multirow{2}{*}{CSQA} & GPT4   & 0.96 & 0.87 & \multirow{2}{*}{0.82}\\
 & & ChatGPT & 0.97 & 0.72 & \\
\cline{2-6}
& \multirow{2}{*}{SocialIQA} & GPT4 & 0.89 & 0.72 & \multirow{2}{*}{0.83}\\
 & & ChatGPT  & 0.98 & 0.70 & \\
\cline{2-6}
 & \multirow{2}{*}{HellaSwag} & GPT4   & 0.96 & 0.87 & \multirow{2}{*}{0.78}\\
 & & ChatGPT & 0.85 & 0.79 & \\
\cline{2-6}
 & \multirow{2}{*}{PIQA} & GPT4   & 0.99 & 0.92 & \multirow{2}{*}{0.92}\\
 & & ChatGPT  & 0.97 & 0.82 & \\
\cline{2-6}
& \multirow{2}{*}{$\alpha$NLI/$\alpha$NLG} & GPT4  & 0.97 &  0.80 & \multirow{2}{*}{0.87}\\
 & & ChatGPT  & 0.91 & 0.70 & \\
\hline
 
 \multirow{4}{*}{NLI} & \multirow{2}{*}{WaNLI} & GPT4   & 0.73 &  0.63 & \multirow{2}{*}{0.70}\\
 & & ChatGPT & 0.62 & 0.43 & \\
 \cline{2-6}
& \multirow{2}{*}{$\delta$-NLI} & GPT4   & 0.89 &  0.92 & \multirow{2}{*}{0.96}\\
 & & ChatGPT  & 0.85 & 0.75 & \\
\hline
 \end{tabular}
\caption{For the negative examples, this table has the aggregated results over hard, medium and easy: \nouha{reporting the hard negative for the discriminative accuracy, will add another table to show the difference between hard and easy. Hard and easy are not applicable for all the tasks, this is why I moved it to a new table.} \faeze{I think having a pot similar to figure \ref{fig:disc_colllie} with their generative vs discriminative performance next to each other is nice and makes the comparison easier. I can do that if you agree on having plots  } \nouha{Good idea, was thinking of that as well. Just having this table now to get a sense of what we have vs not. For each dataset, we can have 1) GPT4/ChatGPT generative vs Human generative (working on running this) and 2) GPT4/ChatGPT discriminative vs Human discriminative) I will add the plots once the experiment is done.}}
    \label{tab:my_label}
\end{table}





\begin{table}[t!]
    \centering
  \footnotesize
   
\begin{tabular}{ |p{2cm}||p{1.5cm}|p{2cm}| p{2cm} | p{2cm} |}
 \hline
Dataset & Model & Candidate type & Model Disc Accuracy & Human Disc Accuracy\\
\hline
\multirow{6}{*}{FaithDial}  & \multirow{3}{*}{GPT4} & hard & 0.63 & 0.86 \\
 & & med & 0.65 & 0.91  \\
 & & easy & 0.73 & 1 \\ 
 \cline{2-5}
 & \multirow{3}{*}{ChatGPT} & hard & 0.60 & same as GPT4 \\
 & & med & 0.66 &  idem \\
 & & easy & 0.71 &  idem \\ 
\hline
\multirow{6}{*}{Topioca}  & \multirow{3}{*}{GPT4} & hard & 0.92 & 0.91 \\
 & & med & 0.95 & 0.92  \\
 & & easy & 0.99 & 0.99 \\ 
 \cline{2-5}
 & \multirow{3}{*}{ChatGPT} & hard & 0.88 & same as GPT4 \\
 & & med & 0.92 &  idem \\
 & & easy & 0.98 &  idem \\ 
\hline
\multirow{6}{*}{XSUM}  & \multirow{3}{*}{GPT4} & hard & 0.19 & 0.84\\
 & & med & 0.82 & 0.88 \\
 & & easy & 0.99 & 0.98\\ 
 \cline{2-5}
 & \multirow{3}{*}{ChatGPT} & hard & 0.10& same as GPT4 \\
 & & med & 0.82 &  idem \\
 & & easy & 1.00 &  idem \\ 
\hline

 \end{tabular}
 \caption{Ablation: measuring the effect of the hardness of the candidates on the performance of the models and humans. }
    \label{tab:my_label}
\end{table}

 








\paragraph{Human Study}
In the human study, we compare human performance setting versus machine performance. The gap between generative and discriminative is more apparent when the candidates are hard. But overall, the gap is not very big  

\paragraph{Human Generation quality vs Machine generation quality}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/human_comparative.png}
\caption{Human comparative study. \nouha{Will improve these plots, but we can see now across all language tasks that humans tend to prefer machine generated answers for both GPT4 and ChatGPT.}}
\label{fig:human_comparative_study}
% \vspace{-8pt}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/generation_discrimination.png}
\caption{Generation vs Discrimination \peter{Love this figure so much! I'm assuming this is using the stand-in numbers on the spreadsheet for now, but I would guess human generative numbers will look a lot like this!} \nouha{Yes, I used the numbers we collected from human eval, each dot corresponds to a task. Another analysis I can do is computing the correlation between models providing correct responses in generation tasks compared to discrimination tasks. While we could apply a similar approach to humans based on the evaluations we're gathering, this correlation may not be entirely fair, as workers responsible for discrimination assessments are not the same ones who generated the responses. } \faeze{This is a very nice figure. Peter and I were thinking on sth similar with Y-axis being comparative perf. and Y-axis being disc. This is much better if we get all results from human generative perf. I have just one concern and that's the discriminative performance for both models and humans are based on ground-truth labels which we are currently evaluating. Maybe we can think of how to avoid complaints? }}
\label{fig:generation_discrimination}
% \vspace{-8pt}
\end{figure}



% \begin{table*}[t]
% \scriptsize
% \centering
% \begin{tabular}{l | l  l  l | l }
%  \toprule

%   \bottomrule
% \end{tabular}
% \caption{\small Human Generation quality vs Machine generation quality}
% \label{tab:human_eval}
% \end{table*}











\subsection{Models can’t even explain their own generations}
In this section, we investigate how models struggle to provide meaningful answers for their own generation.  While models often excel at generating accurate answers based on provided background information, they face difficulties when questioned about their own generation. To investigate this phenomenon, we conduct a cyclic evaluation comprising two steps: First, we task the models with generating a paragraph using specific background information. Second, we pose questions to the models regarding their own generated content, aiming to assess their comprehension and self-awareness.  

Talk about the tasks: 1) Reading comprehension, 2) physical reasoning and 3) Collie







\subsection{Probing Model's [Understanding?] on [of] their Generations}

\faeze{WIP}
\begin{figure}[th]
    \centering
\includegraphics[scale=0.3]{figures/generative_collie.pdf}
    \caption{Constraint Satisfaction of GPT-3.5 (left) and GPT-4 (right) Generations on Collie Benchmark \cite{}.}
    \label{fig:gen_collie}
\end{figure}

\begin{figure}[th]
    \centering
\includegraphics[scale=0.25]{figures/discriminative_collie_v2.pdf}
    \caption{Accuracy of GPT-3.5 (left) and GPT-4 (right) on understanding the correctness of their own generations. \faeze{still need to add values to these plots.} \faeze{Presenting these two sets of plots (gen and disc) separately might not be ideal. Any suggestion to improve? We can also show all accuracies (gen accuracy, disc on correct gen, disc on incorrect gen, and dics overall) together. wdu?} \peter{Thinking about this. I think it would be good to highlight the kinds of mistakes the model would make. e.g. for word02, it looks like the accuracy in telling that the answer is incorrect is actually quite low? So I'm assuming this means it's likely that the understanding model would say that some of the incorrect generations are correct? But this takes some time to recognize with plots in their current form. Also depends on whether we are framing exp2 as ``understanding of their successful gens'' or more generally just ``model understanding of their own generations (by QA)''} \faeze{Yeah, in word02 none of the generations where successful and understanding model where only able to identify few of them. I think understanding models' generation in general would be safer than just their successful one just because the reviewer might ask why didn't you look into that}}
    \label{fig:disc_colllie}
\end{figure}



==> sections/history/3_experiments_v2.tex <==
% \section{Exploring the Duality of Language and Vision Models: Generation vs. Understanding }
\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figures/language/chatgpt_human_disc_gen_v2.pdf}
    \includegraphics[width=\linewidth]{figures/language/results_figure.pdf}
    \caption{\small{Human evaluation results of ChatGPT vs. human performances under the generative and discriminative task formulation.
    }}
    \vspace{-15pt}
    \label{fig:chatgpt_exp1_language}
\end{figure}






% . \nouha{condense the following paragraph to talk about evaluation. }

% For the generative setting, we conduct human evaluations on AMT to judge whether the generated image matches the text prompt. To better mimic the user scenario of Midjourney, we consider 4 output images per prompt and report the successful rates per prompt (\textit{i.e.}, we regard a success when at least one of the four images matches the text prompt). 

% \nouha{move this to the ablation study section}
% For the discriminative setting, we take the subset of text prompts that Midjourney have at least one successful generation, and construct the candidate pairs with a successful generation and a failed generation. \nouha{We don't need to discuss details on how we construct candidates here, this can be move to appendix. We can just mention the overall task. }
% To verify the feasibility of these discriminative samples, we again sort to AMT and only retain the samples with agreeable answers among 3 workers. In real user scenario of image generation models, the image selection step, which requires understanding on the generated images, is usually conducted by human.   We consider \textbf{CLIP}~\cite{} and \textbf{Open-CLIP}~\cite{} models for discriminative evaluation, as they are trained to measure the similarity between image and text, and test whether manual image selection can be replaced by image understanding models.  Here, Similarly, we report accuracy as the evaluation metric for the discriminative setting. 
% See details of AMT annotations and instructions on vision experiments in \S~\ref{}.
% \lindsey{I included much more detail in how we setup discriminative setting for vision experiments here. Feel need to explain before presenting the results.}








% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/language/hard_neg_language-cropped.pdf}
%     \caption{\small GPT-4 and human performance across varying levels of answer difficulty. Refer to \S\ref{} for ChatGPT performance. \nouha{include vision, this will be one column figure not a wrapfigure}}
%     \vspace{-10pt}
%     \label{fig:hard_neg_lang}
% \end{figure}







% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/vision_gen_disc.png}
% \caption{Vision generation models performance and understanding models discrimination performance. \nouha{Don't consider aesthetics for now, will improve it}}
% \label{fig:midjourney accuracy}
% \vspace{-5pt}
% \end{figure}

\section{Do models' generation exceed selective understanding?}
\label{sec:exp1}

%\peter{Could consider a question for the title like ``Does model generation outpace selective understanding?'' and kind of leave the \emph{human} aspect implicit (we cover it in section 2) or maybe have a super short paragraph at the beginning to reiterate the subhypothesis} \nouha{feel free to edit}
%\pw{what is selective understanding? it didn't appear in section 2, so perhaps keep the terminology consistent? (likewise, it would help if we used the same verbs as in the hypothesis, as in exceed vs.~outpace}

%\ake{Based on new framing as discussed earlier, transition now something like ``In this section we ask the question: given a generation problem, how does models' ability to generate a correct answer compare to their ability to select from among a set of candidate answers?'' (Peter refine to make consistent)}
%\peter{Will experiment with below paragraph}

In this section, we analyze models' generation and understanding capabilities via a side-by-side analysis of performance on generative and discriminative variants of tasks, and we compare this performance to that of humans. We make these comparisons for both language and vision models, drawing on diverse benchmarks. %, and adapting those tasks to have parallel generative and discriminative versions. 
We list these source benchmarks below:

\paragraph{Language Benchmarks} In the dialogue domain, we explore open-ended datasets namely \textbf{Mutual}$^+$ \citep{cui-etal-2020-mutual} and \textbf{DREAM} \citep{sun-etal-2019-dream}, and a document-grounded benchmark, \textbf{Faithdial} \cite{dziri2022faithdial}. These require generating coherent continuations based on conversation history (faithful to the document in grounded dialogue). For reading comprehension, we include \textbf{Topioca} \citep{adlakha2022topiocqa} (conversational QA) and \textbf{RACE} \citep{lai-etal-2017-race} (factual QA). % and  \textbf{Vitamin 
For summarization, we consider \textbf{XSUM} \citep{narayan-etal-2018-dont}. We include multiple commonsense benchmarks:  \textbf{CommonSenseQA} \citep{talmor-etal-2019-commonsenseqa}, \textbf{SocialIQA} \citep{sap-etal-2019-social}, \textbf{HellaSwag} \citep{zellers-etal-2019-hellaswag}, \textbf{PIQA} \citep{seo2018phrase}, \textbf{$\alpha$NLG/$\alpha$NLI} \citep{bhagavatula2020abductive}. Lastly, we considered NLI tasks \textbf{WaNLI} \citep{liu-etal-2022-wanli}, and \textbf{$\delta$-NLI} \citep{rudinger-etal-2020-thinking}.


\paragraph{Vision Benchmarks} For image generation, we use four benchmarks for text prompts, from descriptions of natural scenes, (likely in-domain for the model), to out-of-distribution scenes with specific attributes and relationships that rarely exist in real images. Prompts are sourced from: \textbf{COCO}~\citep{lin2014microsoft}, \textbf{PaintSkill}~\citep{Cho2022DallEval}, \textbf{DrawBench}~\citep{saharia2022photorealistic} and \textbf{T2ICompBench}~\citep{huang2023t2icompbench}. See Appendix \S\ref{app_models_dataset} for more dataset details.

\paragraph{Experimental Setup} For each task in both modality, we consider two settings: \textbf{i) generative:} we prompt models to generate a response given task-specific inputs (e.g., dialogue history, document, premise, image caption, etc.)%For generating textual responses, we use ChatGPT and GPT4 and for generating images, we prompt Midjourney with textual captions. 
, and \textbf{ii) discriminative:} we require task-specific models to select the correct answer from a set of candidates, using existing candidates where available and otherwise generating options. (see Appendix \S\ref{app_negative_examples} for details).
%\faeze{We use available candidates in the datasets that are originally designed as multiple-choice. Whereas, we automatically create candidates for tasks that are originally generative (e.g.,, summarization) (see Appendix \S\ref{app_negative_examples} for details).} \lindsey{can I just point to 3.2 on how to construct candidates for vision?}
 %\footnote{For language-related tasks, we use ChatGPT and GPT4 for choosing a response from 4 candidates. For vision, we require the image understanding models (i.e., CLIP, OpenCLIP) to select the image that better matches the textual description from two candidates}. 
% Within language, we use GPT-4 and Chat-GPT as both generation and understanding models. In the vision domain, we use Midjourney for the generation and understanding models (i.e., CLIP, OpenCLIP) for discrimination. % \ben{Do we need to repeat this :thumbsup:}\faeze{yeah I see we have it up there and I think we can skip this. I just tried to rephrase how it was presented here. }
 
% Evaluation metrics are consistent across modalities.
For the generative setting, we conduct human evaluations using Amazon Mechanical Turk (AMT) to judge the correctness of responses (i.e, text or image) and report percentage of successful responses satisfying task requirements. For the discriminative setting, we report the accuracy of choosing the ground-truth response among the candidate options.  
To establish a human performance baseline, we ask workers to perform all discriminative tasks, and to evaluate correctness of the ground truth responses for each task.\footnote{Ground truth responses were initially written by humans.} %which was initially generated by humans. 
Details of AMT annotations and instructions are in \S\ref{app:human_eval_details}.%\lasha{We should describe how we get the candidates for the discriminative setting.}

% we ask humans to judge the discrimination task and do rate the groundtruth response



 % For the generative setting, we conduct human evaluations on AMT to judge whether the generated image matches the text prompt.



\subsection{Generative and discriminative capabilities in models vs.~humans}
% \pw{to fit in the same line,
% generative and discriminative capabilities in models vs.~humans?}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/vision/vision_exp1_v2.png}
    \caption{
    % \peter{We should probably explicitly label generative/discriminative in the legend or bars themselves, to make it obvious that we're comparing these two different settings}\lindsey{added, also fixed the one for vision exp2.}
    \small{Model and human performance under the generative and discriminative settings on vision modality.}}
    % Intuitively, we expect generative performance for an average human to be much poorer than image generation model (\emph{i.e.}, Midjourney).}}
    \label{fig:vision-expt1-main-results}
    \vspace{-15pt}
\end{figure}

\footnotetext{
We report the best results on CLIP (\texttt{clip-vit-large-patch14}) and OpenCLIP (\texttt{CLIP-ViT-bigG-14-laion2B-39B-b160k}), more results can be found in \S\ref{}.}




\paragraph{Language.} Figure~\ref{fig:chatgpt_exp1_language} presents a comparison of ChatGPT and GPT4 generative and discriminative performance with that of humans.
% are presented.
% {fig:expt1-main-results-v2},
% The results show a complex landscape reflecting varied performance across different tasks and configurations. 
% However, 
Two clear trends emerge from the results: First, the model's generative accuracy regularly exceeds that of the humans, but the discriminative accuracy never does. Second, more often than not, the model's generative accuracy exceeds its discriminative accuracy. Figure~\ref{fig:disagreement_gpt4} illustrates this divergence more closely in GPT-4's performance\footnote{The same trend applies for ChatGPT (See \S\ref{generation_vs_discrimination})}.
% between generation and discrimination. 
For instance, in the XSUM task, GPT-4 generates a correct summary in 34\% of cases but fails to choose the correct summary from a list of options for the same examples.
This begs the question: if models can generate the correct answer, why do they encounter difficulties in selecting it?  This behavior contradicts that of humans. Figure~\ref{fig:chatgpt_exp1_language} shows that if humans have the capability to generate the right response, they often exhibit comparable proficiency in selecting the correct answer (from the candidates) % from a predefined list 
which is not the case for models--- GPT-4's high generative performance does not consistently translate into high discriminative performance.  
% \ake{This is also another analysis which should get a clearer transition. Is there a reason we have this for GPT-4 and not ChatGPT? Can we be more clear/consistent with choice of models/analyses/comparisons?} \nouha{We have the same results for GPT4 and ChatGPT} Figure~\ref{fig:gpt4_disc_gen} further illustrates this contrast: while humans show a positive correlation between their discrimination and generation abilities,


\begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-5pt}
\includegraphics[width=\linewidth]{figures/language/agreement_gpt4-cropped.pdf}
\vspace{-18pt}
\caption{\small{GPT-4's discrepancy: accurate generation but inaccurate selection for the same example.}}
% \vspace{-26pt}
\label{fig:disagreement_gpt4}
\end{wrapfigure}



\begin{figure}[t!]
\captionsetup[subfloat]{farskip=1pt,captionskip=2pt}
\centering
   \subfloat[\small{GPT-4 vs. human.}]{
      \includegraphics[width = 0.485\columnwidth]{figures/language/lang_neg.pdf}\label{fig:hard_neg_lang}
   }\hfill
   \subfloat[\small{OpenCLIP vs. human.}]{
      \includegraphics[width = 0.485 \columnwidth]{figures/vision/vision_neg.pdf}\label{fig:hard_neg_vision}
   }
   \vspace{-5pt}
   \caption{
    \small{ Model and human performance across varying levels of answer difficulty.}
   }
    \vspace{-10pt}
    \label{fig:hard_neg}
\end{figure}

% Intuitively, humans are expected to have much lower performance in generating high-quality images compared to Midjourney \ake{not sure you should include that speculation---maybe humans can't produce beautiful images like Midjourney, but they probably wouldn't be inaccurate in their stick figures or whatever they can produce.}. \nouha{I agree, not sure how to talk about this tbh}

\paragraph{Vision.} When evaluating vision models, it is not practical to ask humans to produce detailed images akin to those generated by image generation models. However, anecdotally we can assume that average humans would not be able to achieve the stylistic quality of models like Midjourney, so we operate under the assumption that generation quality in humans is lower. As a result, we only compare models' generative and discriminative accuracy to humans' discriminative accuracy. Similar to the language domain, Figure~\ref{fig:vision-expt1-main-results} shows 
% Intuitively, average humans are expected to have much lower performance in generating lifelike images compared to Midjourney. This observation holds true even if the prompt does not explicitly demand lifelike images. Models possess the capability to produce such images, whereas the average human may struggle to achieve the same level of visual fidelity.
%As in the language domain, we see again 
that models fall short of human accuracy in discriminative performance. However, unlike the language domain, we find that vision models' generative accuracy actually falls short of the discriminative accuracy %, by contrast to the language domain.  
This suggests that the dazzling impressions of generative image models may be driven more by stylistic quality in model generations, than by generative correctness.
 % This phenomenon suggests that the images produced by these models are more notable for their stylistic quality than for their accuracy in faithfully generating the intended content.
% Models may occasionally produce images that deviate from the provided caption, but their impressive stylistic quality can often overshadow these inaccuracies. 
People tend to be so impressed by the visual appeal that they may not pay as much attention to the occasional mistakes.


% \nouha{not sure about the conclusion here.} \nouha{Allyson said "This phenomenon implies that the image outputs generated by these models are more remarkable for their visual quality than for their accuracy." but not sure if I follow this }
% Interestingly, we note that humans excel in discrimination compared to vision understanding models like CLIP and OpenCLIP. In contrast, vision models surpass human capabilities when it comes to generating images. This pattern mirrors the observations in language-related tasks, where models excel in generation but fall behind humans in discrimination tasks.



% We observe similar trends to the ones in language modality, that is image understanding models lag behind human on discriminative performance, while image generation models are better at generations than human.  

% In certain contexts, humans may encounter difficulties when attempting to articulate their thoughts or generate text or images in response to a question. However, when provided with a structured set of answer options, they often succeed at choosing the accurate response [mention the vision experiments].


%% what's the story to tell
% 1- Models are better at generation than discrimination
% 2- There is an inconsistency in models when answering the same question: They can provide a correct answer in the generative mode but at the same time fail to provide a correct answer in the discriminative mode. This is a paradox, if you're able to produce the right answer, why do you struggle to select it. Contrast this to humans where humans are most likely able to choose the right answer among candidates if they're able to generate a correct answer without being asked to choose from a list. The other way can be understandable in human behavior, when humans don't know how to generate 
% Talk about how the models' quality of generated responses is prefered over humans: explain the reasons and 



% \begin{figure}
% \setlength{\belowcaptionskip}{-.5\baselineskip}
% \setlength{\abovecaptionskip}{0.3\baselineskip}
% \centering
%     % \vspace{-2em}
%     % \hfill
%    \begin{minipage}[t]{0.4\textwidth}
%      \centering
% \includegraphics[width=\linewidth]{figures/language/gpt4_disc_gen-cropped.pdf}
%    \end{minipage}
%    \begin{minipage}[t]{0.5\textwidth}
%      \centering
% \includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}
%    \end{minipage}
%     \caption{(a) \small \textbf{}. (b) \textbf{} 
%     }
%     \label{fig:zero-shot}
%     %\vspace{-3mm}
% \end{figure} 






% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/vision_gen_disc.png}
% \caption{Vision generation models performance and understanding models discrimination performance. \nouha{Don't consider aesthetics for now, will improve it}}
% \label{fig:midjourney accuracy}
% \vspace{-5pt}
% \end{figure}







\subsection{Models fall further short of human performance with harder discrimination tasks}

% \nouha{open also for ``How does candidate hardness affect the generation-discrimination gap?''}
% \ake{IF using the title to report results, maybe ``Models fall further short of human humans with harder discrimination tasks''} \peter{Or maybe a question ``How does candidate hardness affect the generation-discrimination gap?'' Then keep the section description pretty short}

% \ake{and start with something like: ``In this section we take a closer look at the gap in discirminative performance between humans and models, by ...''}

% \peter{We probably also want to compress this section as it is only a subpart of experiment 1.}

\lindsey{We could potentially move negative setting details to appendix, and only discuss the sub-figures under language and vision paragraph. and start the section with:} We take a closer look at the gap in discriminative performance between humans and models, by manipulating the difficulty of the negative candidates\footnote{Refer to \S\ref{app_negative_examples} for details about the negative candidates construction}. Results are shown in Figure~\ref{fig:hard_neg}.


\paragraph{Language}
We take a closer look at the gap in discriminative performance between humans and models, by manipulating the difficulty of the candidate options. 
For tasks originally designed to be generative (i.e., FaithDial and XSUM), we construct a candidate set $N$ comprising $N-1$ negative candidates and the ground-truth answer.  
% To generate the negative answers, we consider 
Three types of negatives are considered: \textbf{i) Hard negatives}:  these are particularly challenging examples 
% designed to make it difficult for 
so that models cannot rely on data biases and artifacts to produce an answer. They contain subtle incorrect information that challenges the models to recognize the errors unless they possess a profound understanding of the task. \textbf{ii) Moderately hard negatives}: these candidates are semantically close to the groundtruth answer, but with errors more noticeable for the models.
And \textbf{iii) Easy negatives}: these candidates are semantically distant from the topic of the question, providing a clear contrast to the correct answer \footnote{Refer to \S\ref{app_negative_examples} for details about the negative candidates construction on language modality.}.

Figure~\ref{fig:hard_neg_lang} shows the comparison between GPT4 and human
% the discriminative performance of GPT4 in discerning answers from a spectrum of difficulty levels among candidate options 
\footnote{See \S\ref{generation_vs_discrimination} for ChatGPT performance.}.  Notably, as the complexity of the candidate answers increases, the model performance shows a gradual decline. For instance, in the XSUM task, GPT4 achieves 100\% accuracy when selecting the correct answer from easy negatives,
% from an array of easy negatives,
but this accuracy drops significantly to 19\% when confronted with hard negatives. It's worth mentioning that XSUM 
exhibits a substantially different performance 
% appears to exhibit a substantial difference in performance 
compared to FaithDial. 
Upon manual inspection, we observed that models tend to make the most mistakes in discrimination tasks when the responses are lengthy and challenging, such as summarizing lengthy documents.
In contrast, human can maintain a consistently high level of accuracy across different levels of difficulty.
% In stark contrast,  human performance exhibits far less variability across different levels of difficulty, maintaining a consistently high level of accuracy.
% \ake{save this summary of implications for end of the section (after vision results) and probably just concisely say the results suggest that humans' disciminative capabilities are both better and more robust to adversarial examples}
%To evaluate the quality of responses for the generative setting, we hire workers from Amazon Mechanical Turk (AMT) (See details in Appendix \S\ref{}). In the discriminative setting, we measure the accuracy of the models choosing the groundtruth answer.

\paragraph{Vision.} 
% To examine the discriminative performance gap of image understanding models across different difficulty levels, 
We similarly construct hard and easy negatives in the image space to evaluate image understanding models \footnote{Constructing moderately hard negatives in the image space is not feasible without reliable image editing tool.\lindsey{not very confident about this reason, maybe we should just remove it. @nouha}}. \textbf{i) Hard negative}: a negative image that is generated based on the same text prompt as the positive image, such that it is semantically close to the text prompt, but contains subtle mistakes.
% identifiable by humans. 
% We  use AMT to verify the feasibility of these hard negative samples and only retain the ones with agreeable judgments among 3 workers. 
\textbf{ii) Easy negative}: a negative image that is randomly sampled from the successful generations of a different prompt in the same dataset as the positive image, such that it is semantically distant from the positive image, hence can be easily distinguishable.  
% In this setting, the negative image would be semantically distant from the positive image, and hence can be easily distinguishable. 



% For the discriminative setting, we take the subset of text prompts that Midjourney have at least one successful generation, and construct the candidate pairs with a successful generation and a failed generation. \nouha{We don't need to discuss details on how we construct candidates here, this can be move to appendix. We can just mention the overall task. }
% In real user scenario of image generation models, the image selection step, which requires understanding on the generated images, is usually conducted by human.   We consider \textbf{CLIP}~\cite{} and \textbf{Open-CLIP}~\cite{} models for discriminative evaluation, as they are trained to measure the similarity between image and text, and test whether manual image selection can be replaced by image understanding models.  Here, Similarly, we report accuracy as the evaluation metric for the discriminative setting. 
Figure~\ref{fig:hard_neg_vision} shows the discriminative performance of OpenCLIP, in comparison to human, across different difficulty levels. 
Consistent with the language results, and even more robustly across task, we see that while human can attain a versatile performance across hard and easy negative settings, model performance drop substantially when confronted with hard negatives (from 100\% to $\sim$69\%). 


 Overall, these results highlight that humans possess the ability to discern the correct answer, even when faced with challenging or adversarial examples, a capability that does not seem to be as robust in LMs. This discrepancy raises fundamental questions about the true extent of these models' understanding, even in relatively simple tasks.

\begin{figure}[t]
   \begin{minipage}[t]{0.4\textwidth}
     \centering
%\includegraphics[width=\linewidth]{figures/exp_mul/average_frequency_of_subgraph_in_training_data.png}
\includegraphics[width=\linewidth]{figures/language/gpt4_disc_gen-cropped.pdf}
\vspace{-22pt}
\caption{\small GPT4 vs Humans. Humans show a larger positive correlation between their discrimination and generation abilities compared to GPT4. \ben{What do the shaded areas inside the dotted lines represent?}}
\label{fig:gpt4_disc_gen}
   \end{minipage}
   \hfill 
   \vspace{3mm} 
      \begin{minipage}[t]{0.5\textwidth}
     \centering
%\includegraphics[width=\linewidth]{figures/exp_mul/error_type.pdf}
%\includegraphics[width=0.9\linewidth]{tmp_figures/figure 5 thinner.pdf}
\includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}

\caption{\small Quality scores of human-generated responses vs. GPT4 response scores}



%Each curve represents the ratio of \textit{all} nodes appearing at the $i$-th layer of some ground truth computation graph that belong to a specific category. 
%This ratio is taken over all computation graphs up to \mel{ASK XIMING}. \nouha{remove in-distribution, ood, and replace those with the puzzzle.}
\label{fig:human_gpt4_comparative}
   \end{minipage}
   \vspace{-7mm}
\end{figure}



\subsection{Models' generations are preferred over Humans generations}
To understand better the gap between humans and LLMs, we asked AMT workers to provide their preferences between machine-generated answers and humans-generated answers, along with the rationale behind their choices \footnote{See \S\ref{app:human_eval_details} for AMT annotation details.}. While both sets of responses score high in correctness, Figure~\ref{fig:human_gpt4_comparative} illustrates a notable trend: workers often favor responses from GPT4 and ChatGPT over those generated by humans. 
Consistent with the observation in section 3.1 (vision), this suggests that models' impressiveness to humans may rely more on aspects like style than on actual accuracy or understanding of content.
\nouha{Talk about the reasons for their preferences. Liwei will provide this Figure by Sep 25th }
This preference for model-generated content is intriguing, considering that LLMs may not possess the same level of genuine understanding and selective accuracy as humans, raising questions about the underlying reasons for these preferences.

% \begin{table}[t!]
%     \centering
%   \footnotesize
%     \input{tables/exp1_results}
%      \caption{Caption:  \liwei{working on a plot on this. To be done by EOD Sept 22}}
%     \label{tab:my_label}
% \end{table}






% \begin{table}[t!]
%     \centering
%   \footnotesize
   
% \begin{tabular}{ |p{2cm}||p{1.5cm}|p{2cm}| p{2cm} | p{2cm} |}
%  \hline
% Dataset & Model & Candidate type & Model Disc Accuracy & Human Disc Accuracy\\
% \hline
% \multirow{6}{*}{FaithDial}  & \multirow{3}{*}{GPT4} & hard & 0.63 & 0.86 \\
%  & & med & 0.65 & 0.91  \\
%  & & easy & 0.73 & 1 \\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.60 & same as GPT4 \\
%  & & med & 0.66 &  idem \\
%  & & easy & 0.71 &  idem \\ 
% \hline
% \multirow{6}{*}{Topioca}  & \multirow{3}{*}{GPT4} & hard & 0.92 & 0.91 \\
%  & & med & 0.95 & 0.92  \\
%  & & easy & 0.99 & 0.99 \\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.88 & same as GPT4 \\
%  & & med & 0.92 &  idem \\
%  & & easy & 0.98 &  idem \\ 
% \hline
% \multirow{6}{*}{XSUM}  & \multirow{3}{*}{GPT4} & hard & 0.19 & 0.84\\
%  & & med & 0.82 & 0.88 \\
%  & & easy & 0.99 & 0.98\\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.10& same as GPT4 \\
%  & & med & 0.82 &  idem \\
%  & & easy & 1.00 &  idem \\ 
% \hline

%  \end{tabular}
%  \caption{Ablation: measuring the effect of the hardness of the candidates on the performance of the models and humans. }
%     \label{tab:negative_candi_results}
% \end{table}

 

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/language/agreement_gpt4-cropped.pdf}
% \caption{Agreement and disagreement between generative and discriminative performance. \liwei{working on refining the plot on this. To be done by EOD Sept 22}}
% \label{fig:agreement}
% % \vspace{-8pt}
% \end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/matrix.png}
% \caption{Agreement and disagreement between generative and discriminative performance (XSUM).}
% \label{fig:agreement}
% % \vspace{-8pt}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/chatgpt_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigure to include them together}}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}
% \caption{GPT4 vs Human comparative study.}
% \label{fig:human_comparative_study}
% % \vspace{-8pt}
% \end{figure}



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/human_comparative.png}
% \caption{Human comparative study. \nouha{Will improve these plots, but we can see now across all language tasks that humans tend to prefer machine generated answers for both GPT4 and ChatGPT.}}
% \label{fig:human_comparative_study}
% % \vspace{-8pt}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/gpt4_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigures to include them together. We can also separate by task categories} \faeze{the gap decreases as models get stronger}}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/chatgpt_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigure to include them together}}
%     \label{fig:enter-label}
% \end{figure}


% \begin{table*}[t]
% \scriptsize
% \centering
% \begin{tabular}{l | l  l  l | l }
%  \toprule

%   \bottomrule
% \end{tabular}
% \caption{\small Human Generation quality vs Machine generation quality}
% \label{tab:human_eval}
% \end{table*}






% \subsection{Models Can’t Explain their Own Generations}
% \section{Probing Models' Understanding of their Generations} 
\section{Can Models Understand What They Generate?}
\label{sec:exp2}

% \peter{May want to swtich the word ``probe'' to avoid other associations/existing definitions. Or possibly change sec title to match \S3? e.g. Can AI understand model generations?}

% \faeze{to be consistent with the question-style of sect 3 and Pang wei's suggestion, we can also have this as: "Can Model Understand what it Generates?"} 

%\ake{Based on new framing as discussed earlier, transition now something like ``In the previous section we formulated understanding as ability to select among a space of possible answers for a task, by contrast to ability to generate a single correct answer. In this section, we take a different angle on understanding: given a generated output, can models accurately answer questions about (the content, appropriateness, etc) of that output?'' (Peter refine to make consistent)}


% \begin{figure}[t!]
% \captionsetup[subfloat]{farskip=1pt,captionskip=2pt}
% \centering
%    \subfloat[\small{GPT-4 performance on generation and question answering based on its own output, versus human’s performance on question  answering based on GPT-4’s output.}]{
%       \includegraphics[width = 0.45\columnwidth]{figures/language/interrogative_exp2_gpt4.pdf}\label{fig:lang-expt2-main-results}
%    }\hfill
%    \subfloat[\small{Model versus human performance on
% visual question answering based on generated images}]{
%       \includegraphics[width = 0.485 \columnwidth]{figures/vision/vision_exp1_v3.png}\label{fig:vision-expt2-main-results}
%    }
%    \vspace{-5pt}
%    \caption{
%     \small{ Results on cyclic evaluation.}
%    }
%     \vspace{-10pt}
%     \label{fig:exp2-cyclic}
% \end{figure}

In the previous section, we show that models often excel at generating accurate answers while lagging behind humans in terms of discriminating answers. % \ake{update that conclusion phrasing if needed for latest version of prior section} \nouha{this is valid only for language}. % In this section, we investigate how models struggle \faeze{this is not true about collie which is very constrained gen task} to provide meaningful understanding of their own generation. 
In this section, we investigate to what extent models can demonstrate meaningful understanding of their own generations, something humans tend to be capable of. We probe models under two different settings: \textbf{(i) cyclic evaluation} (\S \ref{cyclic_probe})  \textbf{(ii) self-reflection} (\S \ref{self_reflect}). Next, we describe each probing setting in detail.  
%comprising two steps:
% First, we task the models with generating a paragraph using specific background information. Second, we pose questions to the models regarding their own generated content, aiming to assess their comprehension and self-awareness.  

% Talk about the tasks: 1) Reading comprehension, 2) physical reasoning and 3) Collie

\subsection{Cyclic Evaluation}
\label{cyclic_probe}
 %\faeze{should we switch probing?}

% \begin{figure}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/language/language_cyclc.pdf}

%     \includegraphics[width=0.9\linewidth]{figures/language/interrogative_exp2_horizental.pdf}
%     % \vspace{-15pt}
%     \caption{\small{In language modality, model's performance on generation and question answering based on its own output, versus human's performance on question answering based on model's output.}}
%     \label{fig:lang-expt2-main-results}
%     % \vspace{-20pt}
% \end{figure}


\paragraph{Language} In cyclic evaluation, we first prompt models to generate a paragraph taking into account some background information, then ask the model multiple-choice questions based on this information using the generation as context.
We perform cyclic evaluation across several benchmarks, including \textbf{XSUM} \citep{narayan-etal-2018-dont} (summarization), \textbf{Mutual}$^+$ \citep{cui-etal-2020-mutual} (dialogue), and \textbf{HellaSwag} \citep{zellers-etal-2019-hellaswag} (commonsense). 

%\ake{In earlier sections we've been contrasting generative vs discriminative with this second section of experiment---but this description sounds like it is also generative vs discriminative, but for the model's own generations rather than arbitrary inputs?} \ximing{}
\input{figures/lang-expt2-main-results}

For \textbf{XSUM}, we prompt the model to generate an article conditioning on a ground-truth summary, and then ask the model to select the best summary for the generated article. \peter{what are the distractors?}
For \textbf{Mutual}$^+$, we prompt the model to generate the conversation history that leads to a given dialogue, and then request the model to choose the best dialogue continuation that history.
For \textbf{HellaSwag}, the model first generates the context preceding a given sentence, and then ask the model to select the most fitting continuation for that generated context. 
We report the model's generation performance, the selection performance based on content generated by the model, and human selection performance using the model's generated content. %\ake{We should explain lack of human generation results.}. 
We use zero-shot GPT-3.5 and GPT-4 for all the evaluations. 
%\ake{I think we need to give a clearer argument for why asking the model to choose the better generation is a test of understanding?} 
In effect, we are asking the model to use its own generation to answer simple contextual questions of preference. As an implicit baseline, we assume humans can answer such questions about their own generations with high accuracy, and so refrain from the complex process of eliciting these generation.

Results are shown in Figure \ref{fig:lang-expt2-main-results}. 
We observe that while the models excel at generation, they make frequent errors in identifying their own source information, indicating a lack of understanding.
%\ake{``Models' discriminative accuracy on their own generations also frequently falls short of humans' accuracy, consistent with ( prev section)''} 
Humans, who could not generate such text at the same speed or scale, consistently achieve higher accuracy in QA compared to the model, though questions are about the model's own output.
%The model's performance is also consistently lower than human's performance when answering questions based model's generation. 
%Noticeably, the model's understanding on model's generation  consistently lags behind human's understanding on model's generation desipte that model has the advantage that questions are based on its own generation.
%The model's performance consistently lags behind that of humans when answering questions based on its own generated content. 
We note that the humans in this study are not experts; producing text as sophisticated as the model's output would likely be a significant challenge. We anticipate that the performance gap in understanding one's own generation would widen even more when comparing the model to human experts, who are likely to answer questions about their own generations with near perfect accuracy. %\peter{Lots of conjecture here, we probably have to soften this a bit still}
%After all, experts, with their genuine understanding, should be able to almost perfectly answer questions about their own writing.





%\ximing{work on this now}\faeze{will work with Ximing to incorporate the results}

\input{sections/vision_exp2}

\subsection{Self-reflection Probing: Constrained Generation}
\label{self_reflect}

Here, we focus on a constrained generation task that is compositional and covers diverse generation levels, i.e., word, sentence, paragraph, and passage. To this end, we use a recently introduced benchmark, \textsc{Collie}-v1 \citep{yao2023collie}. \textsc{Collie} contains 2,080 constraint instances across 13 different task types shown in Appendix Table \ref{tab:collie_examples}. \faeze{Given the table goes to appendix do you think we need to give an example of the task in this paragraph? or can it wait to next parag} We zero-shot prompt ChatGPT/GPT-4 to generate outputs for 50 examples per task. We then ask them to reflect on their own generations and verify if they satisfy the given constraints. 


Figure \ref{fig:gpt4_collie_condensed} shows GPT-4 constraint satisfaction rate across 6 representative tasks in Collie (see Appendix Figure \ref{fig:collie_gpt4_full} for full results). Certain tasks with simple constraints such as \texttt{word01} (generating a word with at least x letters), and \texttt{sent04} (generating a sentence containing words A, B, C). %, and \texttt{para01} (generating a paragraph with each sentence starting with word A) are less challenging for models. 
However, we observe significant drop in performance when posed with arbitrary position constraints and strict counting requirements (e.g., \texttt{sent02}, generating a sentence with x words, where the 3rd word is A, and the 7th word is B ...), suggesting that current models cannot handle generations when faced with rich compositional constraints.

\input{figures/collie_condensed_v2}

Figure \ref{fig:gpt4_collie_condensed}, orange bars, show GPT-4 performance at accurately identifying if its own generations satisfy the given constraints. We show the breakdown of discriminative accuracy on all, correct, and incorrect model generations. We observe that GPT-4 generally demonstrates comparable discriminative performance on less challenging tasks. However, for more challenging constrained tasks, discriminative performance surpasses that of generative one. These observations validate our hypothesis that generative and discrminative capabilities are influenced by the constraint levels and open-endedness of the tasks.


% \begin{figure}[th]
%     \centering
% \includegraphics[scale=0.3]{figures/generative_collie.pdf}
%     \caption{Constraint Satisfaction of GPT-3.5 (left) and GPT-4 (right) Generations on Collie Benchmark \cite{}.}
%     \label{fig:gen_collie}
% \end{figure}

% \begin{figure}[th]
%     \centering
% \includegraphics[scale=0.25]{figures/discriminative_collie_v2.pdf}
%     \caption{Accuracy of GPT-3.5 (left) and GPT-4 (right) on understanding the correctness of their own generations.
%     }
%     \label{fig:disc_colllie}
% \end{figure}


\input{figures/disagreement_figure}


==> sections/history/3_experiments_v3.tex <==
% \section{Exploring the Duality of Language and Vision Models: Generation vs. Understanding }
\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figures/language/chatgpt_human_disc_gen_v4.pdf}
    \includegraphics[width=\linewidth]{figures/expt1_main_results_v7.pdf}
    \caption{
    \small{Human evaluation results of ChatGPT vs. human performances under the generative and discriminative task formulation.
    }
    }
    \vspace{-15pt}
    \label{fig:chatgpt_exp1_language}
\end{figure}






% . \nouha{condense the following paragraph to talk about evaluation. }

% For the generative setting, we conduct human evaluations on AMT to judge whether the generated image matches the text prompt. To better mimic the user scenario of Midjourney, we consider 4 output images per prompt and report the successful rates per prompt (\textit{i.e.}, we regard a success when at least one of the four images matches the text prompt). 

% \nouha{move this to the ablation study section}
% For the discriminative setting, we take the subset of text prompts that Midjourney have at least one successful generation, and construct the candidate pairs with a successful generation and a failed generation. \nouha{We don't need to discuss details on how we construct candidates here, this can be move to appendix. We can just mention the overall task. }
% To verify the feasibility of these discriminative samples, we again sort to AMT and only retain the samples with agreeable answers among 3 workers. In real user scenario of image generation models, the image selection step, which requires understanding on the generated images, is usually conducted by human.   We consider \textbf{CLIP}~\cite{} and \textbf{Open-CLIP}~\cite{} models for discriminative evaluation, as they are trained to measure the similarity between image and text, and test whether manual image selection can be replaced by image understanding models.  Here, Similarly, we report accuracy as the evaluation metric for the discriminative setting. 
% See details of AMT annotations and instructions on vision experiments in \S~\ref{}.
% \lindsey{I included much more detail in how we setup discriminative setting for vision experiments here. Feel need to explain before presenting the results.}








% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/language/hard_neg_language-cropped.pdf}
%     \caption{\small GPT-4 and human performance across varying levels of answer difficulty. Refer to \S\ref{} for ChatGPT performance. \nouha{include vision, this will be one column figure not a wrapfigure}}
%     \vspace{-10pt}
%     \label{fig:hard_neg_lang}
% \end{figure}







% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/vision_gen_disc.png}
% \caption{Vision generation models performance and understanding models discrimination performance. \nouha{Don't consider aesthetics for now, will improve it}}
% \label{fig:midjourney accuracy}
% \vspace{-5pt}
% \end{figure}

\section{Do models' generation exceed selective understanding?}
\label{sec:exp1}

%\peter{Could consider a question for the title like ``Does model generation outpace selective understanding?'' and kind of leave the \emph{human} aspect implicit (we cover it in section 2) or maybe have a super short paragraph at the beginning to reiterate the subhypothesis} \nouha{feel free to edit}
%\pw{what is selective understanding? it didn't appear in section 2, so perhaps keep the terminology consistent? (likewise, it would help if we used the same verbs as in the hypothesis, as in exceed vs.~outpace}

%\ake{Based on new framing as discussed earlier, transition now something like ``In this section we ask the question: given a generation problem, how does models' ability to generate a correct answer compare to their ability to select from among a set of candidate answers?'' (Peter refine to make consistent)}
%\peter{Will experiment with below paragraph}

\ake{First, in our \emph{selective} evaluation}  we conduct a side-by-side performance analysis on generative and discriminative variants of tasks to assess models' generation and understanding capabilities in  language and vision modalities. We compare this generative and discriminative performance to that of humans. %, and adapting those tasks to have parallel generative and discriminative versions.
For our tasks we draw on diverse source benchmarks, detailed below:

\paragraph{Language Benchmarks.} In the \textit{dialogue domain,} we explore two open-ended datasets---\textbf{Mutual}$^+$ \citep{cui-etal-2020-mutual} and \textbf{DREAM} \citep{sun-etal-2019-dream}, and a document-grounded benchmark, \textbf{Faithdial} \citep{dziri2022faithdial}. These tasks require the generation of coherent continuations based on conversation history (faithful to the document in grounded dialogue). For \textit{reading comprehension}, we include \textbf{Topioca} (\citealt{adlakha2022topiocqa}; conversational QA) and \textbf{RACE} (\citealt{lai-etal-2017-race}; factual QA). % and  \textbf{Vitamin 
For \textit{summarization}, we consider \textbf{XSUM} \citep{narayan-etal-2018-dont}. We also include multiple \textit{commonsense} benchmarks:  \textbf{CommonSenseQA} \citep{talmor-etal-2019-commonsenseqa}, \textbf{SocialIQA} \citep{sap-etal-2019-social}, \textbf{HellaSwag} \citep{zellers-etal-2019-hellaswag}, \textbf{PIQA} \citep{seo2018phrase}, \textbf{$\alpha$NLG/$\alpha$NLI} \citep{bhagavatula2020abductive}. Lastly, we considered the \textit{NLI tasks} \textbf{WaNLI} \citep{liu-etal-2022-wanli} and \textbf{$\delta$-NLI} \citep{rudinger-etal-2020-thinking}.


\paragraph{Vision Benchmarks.} For image generation, we source text prompts from four benchmarks: these range from descriptions of natural scenes, (likely in-domain for the model) to out-of-distribution scenes with specific attributes and relationships that rarely exist in real images. Prompts are sourced from: \textbf{COCO}~\citep{lin2014microsoft}, \textbf{PaintSkill}~\citep{Cho2022DallEval}, \textbf{DrawBench}~\citep{saharia2022photorealistic} and \textbf{T2ICompBench}~\citep{huang2023t2icompbench}. See Appendix \S\ref{app_models_dataset} for more dataset details.

\paragraph{Experimental Setup.} For each task and modality, we consider two settings: \textbf{i) generative:} we prompt models to generate a response given task-specific inputs (e.g., dialogue history, document, image caption)%For generating textual responses, we use ChatGPT and GPT4 and for generating images, we prompt Midjourney with textual captions. 
, and \textbf{ii) discriminative:} we require task-specific models to select the correct answer from a set of candidates, using existing candidates where available and otherwise generating options. 
% (see Appendix \S\ref{app_negative_examples} for details).
%\faeze{We use available candidates in the datasets that are originally designed as multiple-choice. Whereas, we automatically create candidates for tasks that are originally generative (e.g.,, summarization) (see Appendix \S\ref{app_negative_examples} for details).} \lindsey{can I just point to 3.2 on how to construct candidates for vision?}
 %\footnote{For language-related tasks, we use ChatGPT and GPT4 for choosing a response from 4 candidates. For vision, we require the image understanding models (i.e., CLIP, OpenCLIP) to select the image that better matches the textual description from two candidates}. 
% Within language, we use GPT-4 and Chat-GPT as both generation and understanding models. In the vision domain, we use Midjourney for the generation and understanding models (i.e., CLIP, OpenCLIP) for discrimination. % \ben{Do we need to repeat this :thumbsup:}\faeze{yeah I see we have it up there and I think we can skip this. I just tried to rephrase how it was presented here. }
 
% Evaluation metrics are consistent across modalities.
For the generative setting, we conduct human evaluations using Amazon Mechanical Turk (AMT) to judge the correctness of responses (i.e, text or image) and report percentage of successful responses satisfying task requirements. For the discriminative setting, we report the accuracy of choosing the ground-truth response among the candidate options.  
To establish a human performance baseline, we ask workers to perform all discriminative tasks and evaluate the correctness of the ground-truth responses for each task.\footnote{Ground-truth responses in the datasets were initially written by humans.} %which was initially generated by humans. 
Details of AMT annotations and instructions are in \S\ref{app:human_eval_details}.%\lasha{We should describe how we get the candidates for the discriminative setting.}

% we ask humans to judge the discrimination task and do rate the groundtruth response



 % For the generative setting, we conduct human evaluations on AMT to judge whether the generated image matches the text prompt.



\subsection{Generative and discriminative capabilities in models vs.~humans}
% \pw{to fit in the same line,
% generative and discriminative capabilities in models vs.~humans?}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/vision/vision_exp1_v3.pdf}
    \caption{
    % \peter{We should probably explicitly label generative/discriminative in the legend or bars themselves, to make it obvious that we're comparing these two different settings}\lindsey{added, also fixed the one for vision exp2.}
    \small{Model and human performance under the generative and discriminative settings on \textbf{vision} modality.}}
    % Intuitively, we expect generative performance for an average human to be much poorer than image generation model (\emph{i.e.}, Midjourney).}}
    \label{fig:vision-expt1-main-results}
    \vspace{-15pt}
\end{figure}

\footnotetext{
We report the best results on CLIP (\texttt{clip-vit-large-patch14}) and OpenCLIP (\texttt{CLIP-ViT-bigG-14-laion2B-39B-b160k}), more results can be found in \S\ref{}.}




\paragraph{Language.} Figure~\ref{fig:chatgpt_exp1_language} presents a comparison of \chatgpt, \gptfour, and human generative and discriminative performances. %with that of humans.
% are presented.
% {fig:expt1-main-results-v2},
% The results show a complex landscape reflecting varied performance across different tasks and configurations. 
% However, 
Two clear trends emerge from the results. First, the generative and discriminative accuracy of humans are nearly equivalent, with no significant gap between them. Second, the model's generative accuracy often exceeds its discriminative accuracy. Figure~\ref{fig:disagreement_gpt4} illustrates this divergence in \gptfour's performance more closely \footnote{The same trend applies for \chatgpt (See Appendix \ref{generation_vs_discrimination})}.
% between generation and discrimination. 
For instance, in the XSUM task, \gptfour generates a correct summary in 34\% of cases but fails to choose the correct summary from a list of options for the same examples.
This begs a question that is counterintuitive for humans: if models can generate the correct answer, why do they encounter difficulties in selecting it?  %This behavior contradicts that of humans. 
Figure~\ref{fig:gpt4_disc_gen_v2} shows that if humans have the capability to generate the correct response, they often exhibit comparable proficiency in selecting the correct answer.
This is not the case for models.  %separated this sentence out to highlight
% \ake{This is also another analysis which should get a clearer transition. Is there a reason we have this for GPT-4 and not ChatGPT? Can we be more clear/consistent with choice of models/analyses/comparisons?} \nouha{We have the same results for GPT4 and ChatGPT} Figure~\ref{fig:gpt4_disc_gen} further illustrates this contrast: while humans show a positive correlation between their discrimination and generation abilities,


\begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-5pt}
\includegraphics[width=\linewidth]{figures/language/agreement_gpt4-cropped.pdf}
\vspace{-18pt}
\caption{\small{GPT-4's discrepancy: accurate generation but inaccurate selection for the same example.}}
% \vspace{-26pt}
\label{fig:disagreement_gpt4}
\end{wrapfigure}



% \begin{figure}[t!]
% \captionsetup[subfloat]{farskip=1pt,captionskip=2pt}
% \centering
%    \subfloat[\small{GPT-4 vs. human.}]{
%       \includegraphics[width = 0.485\columnwidth]{figures/language/lang_neg.pdf}\label{fig:hard_neg_lang}
%    }\hfill
%    \subfloat[\small{OpenCLIP vs. human.}]{
%       \includegraphics[width = 0.485 \columnwidth]{figures/vision/vision_neg.pdf}\label{fig:hard_neg_vision}
%    }
%    \vspace{-5pt}
%    \caption{
%     \small{ Model and human performance across varying levels of answer difficulty.}
%    }
%     \vspace{-10pt}
%     \label{fig:hard_neg}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/expt1_lan_vi_hardness_v1.pdf}
    \caption{Model and human performance across varying levels of answer difficulty.}
    % Intuitively, we expect generative performance for an average human to be much poorer than image generation model (\emph{i.e.}, Midjourney).}}
    \label{fig:hard_neg}
    \vspace{-15pt}
\end{figure}



% Intuitively, humans are expected to have much lower performance in generating high-quality images compared to Midjourney \ake{not sure you should include that speculation---maybe humans can't produce beautiful images like Midjourney, but they probably wouldn't be inaccurate in their stick figures or whatever they can produce.}. \nouha{I agree, not sure how to talk about this tbh}

\paragraph{Vision.} When evaluating vision models, it is not practical to ask humans to produce detailed images akin to those generated by image generation models. However, since we can assume that an average human would not be able to achieve the stylistic quality of models like Midjourney, we operate under the assumption that generation quality in humans is lower. As a result, we only compare models' generative and discriminative accuracy to humans' discriminative accuracy. Similar to the language domain, Figure~\ref{fig:vision-expt1-main-results} shows 
% Intuitively, average humans are expected to have much lower performance in generating lifelike images compared to Midjourney. This observation holds true even if the prompt does not explicitly demand lifelike images. Models possess the capability to produce such images, whereas the average human may struggle to achieve the same level of visual fidelity.
%As in the language domain, we see again 
that models fall short of human accuracy in discriminative performance. However, unlike the language domain, we find that vision models' generative accuracy, too, falls short of the discriminative accuracy. %, by contrast to the language domain.  
This suggests that the impressions humans have of models' dazzling generative capability 
%of generative image models 
may be driven more by stylistic quality in model generations, than by generative correctness.
 % This phenomenon suggests that the images produced by these models are more notable for their stylistic quality than for their accuracy in faithfully generating the intended content.
Models may occasionally produce images that deviate from the provided caption, but their impressive stylistic quality and visual appeal can often overshadow these inaccuracies. 
%People tend to be so impressed by the visual appeal that they may not pay as much attention to the occasional mistakes.


% \nouha{not sure about the conclusion here.} \nouha{Allyson said "This phenomenon implies that the image outputs generated by these models are more remarkable for their visual quality than for their accuracy." but not sure if I follow this }
% Interestingly, we note that humans excel in discrimination compared to vision understanding models like CLIP and OpenCLIP. In contrast, vision models surpass human capabilities when it comes to generating images. This pattern mirrors the observations in language-related tasks, where models excel in generation but fall behind humans in discrimination tasks.



% We observe similar trends to the ones in language modality, that is image understanding models lag behind human on discriminative performance, while image generation models are better at generations than human.  

% In certain contexts, humans may encounter difficulties when attempting to articulate their thoughts or generate text or images in response to a question. However, when provided with a structured set of answer options, they often succeed at choosing the accurate response [mention the vision experiments].


%% what's the story to tell
% 1- Models are better at generation than discrimination
% 2- There is an inconsistency in models when answering the same question: They can provide a correct answer in the generative mode but at the same time fail to provide a correct answer in the discriminative mode. This is a paradox, if you're able to produce the right answer, why do you struggle to select it. Contrast this to humans where humans are most likely able to choose the right answer among candidates if they're able to generate a correct answer without being asked to choose from a list. The other way can be understandable in human behavior, when humans don't know how to generate 
% Talk about how the models' quality of generated responses is prefered over humans: explain the reasons and 



% \begin{figure}
% \setlength{\belowcaptionskip}{-.5\baselineskip}
% \setlength{\abovecaptionskip}{0.3\baselineskip}
% \centering
%     % \vspace{-2em}
%     % \hfill
%    \begin{minipage}[t]{0.4\textwidth}
%      \centering
% \includegraphics[width=\linewidth]{figures/language/gpt4_disc_gen-cropped.pdf}
%    \end{minipage}
%    \begin{minipage}[t]{0.5\textwidth}
%      \centering
% \includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}
%    \end{minipage}
%     \caption{(a) \small \textbf{}. (b) \textbf{} 
%     }
%     \label{fig:zero-shot}
%     %\vspace{-3mm}
% \end{figure} 






% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/vision_gen_disc.png}
% \caption{Vision generation models performance and understanding models discrimination performance. \nouha{Don't consider aesthetics for now, will improve it}}
% \label{fig:midjourney accuracy}
% \vspace{-5pt}
% \end{figure}







\subsection{Models fall further short of human performance with harder discrimination tasks}

% \nouha{open also for ``How does candidate hardness affect the generation-discrimination gap?''}
% \ake{IF using the title to report results, maybe ``Models fall further short of human humans with harder discrimination tasks''} \peter{Or maybe a question ``How does candidate hardness affect the generation-discrimination gap?'' Then keep the section description pretty short}

% \ake{and start with something like: ``In this section we take a closer look at the gap in discirminative performance between humans and models, by ...''}

% \peter{We probably also want to compress this section as it is only a subpart of experiment 1.}
We take a closer look at the gap in discriminative performance between humans and models by manipulating the difficulty of the negative candidates. 
Three types of negatives are considered: \textbf{i) hard negatives}:  particularly challenging examples that deter models from relying
% designed to make it difficult for 
%so that models cannot rely 
on data biases and artifacts to produce an answer. The incorrectness in these negatives are subtle and challenging; recognizing these errors may require a profound level of understanding of the task. And \textbf{iii) Easy negatives}: these candidates are semantically distant from the topic of the question, providing a clear contrast to the correct answer.\footnote{Refer to \S\ref{app_negative_examples} for details about the negative candidates construction on language and vision modalities. For the language domain, hard negatives are constructed only for tasks that are originally generative in nature (i.e., FaithDial and XSUM).} 

Figure~\ref{fig:hard_neg_lang} shows the comparison between \gptfour and human
% the discriminative performance of GPT4 in discerning answers from a spectrum of difficulty levels among candidate options 
\footnote{See \S\ref{generation_vs_discrimination} for \chatgpt performance.}.  Notably, as the complexity of the candidate answers increases, the model performance shows a gradual decline. For instance, in the XSUM task, GPT4 achieves 100\% accuracy when selecting the correct answer from easy negatives,
% from an array of easy negatives,
but this accuracy drops significantly to 19\% when confronted with hard negatives. It is worth mentioning that XSUM 
exhibits a substantially different performance 
% appears to exhibit a substantial difference in performance 
compared to FaithDial. 
Upon manual inspection, we observe that models tend to make the most mistakes in discrimination tasks when the responses are lengthy and challenging, such as summarizing lengthy documents.
In contrast, humans can maintain a consistently high level of accuracy across different levels of difficulty.

Figure~\ref{fig:hard_neg_vision} shows the discriminative performance of OpenCLIP, in comparison to human, across difficulty levels. 
Consistent with the language results, and even more robustly across task, we see that while human can attain a versatile performance across hard and easy negative settings, model performance drop substantially when confronted with hard negatives (from 100\% to $\sim$69\%). 
 Overall, these results highlight that humans possess the ability to discern the correct answer even when faced with challenging or adversarial examples. We observe that this capability is not as robust in LMs. This discrepancy raises fundamental questions about the true extent of these models' understanding, even in relatively simple tasks.




% \paragraph{Language}
% For tasks originally designed to be generative (i.e., FaithDial and XSUM), we construct a candidate set $N$ comprising $N-1$ negative candidates and the ground-truth answer.  
% % To generate the negative answers, we consider 
% Three types of negatives are considered: \textbf{i) hard negatives}:  particularly challenging examples that deter models from relying
% % designed to make it difficult for 
% %so that models cannot rely 
% on data biases and artifacts to produce an answer. The incorrectness in these negatives are subtle and challenging; recognizing these errors may require a profound level of understanding of the task.
% %They contain subtle incorrect information that challenges the models to recognize the errors unless they possess a profound understanding of the task.
% % \textbf{ii) moderately hard negatives}: these candidates are semantically close to the groundtruth answer, but with errors more noticeable for the models.
% And \textbf{iii) Easy negatives}: these candidates are semantically distant from the topic of the question, providing a clear contrast to the correct answer \footnote{Refer to \S\ref{app_negative_examples} for details about the negative candidates construction on language modality.}.


% In stark contrast,  human performance exhibits far less variability across different levels of difficulty, maintaining a consistently high level of accuracy.
% \ake{save this summary of implications for end of the section (after vision results) and probably just concisely say the results suggest that humans' disciminative capabilities are both better and more robust to adversarial examples}
%To evaluate the quality of responses for the generative setting, we hire workers from Amazon Mechanical Turk (AMT) (See details in Appendix \S\ref{}). In the discriminative setting, we measure the accuracy of the models choosing the groundtruth answer.

% \paragraph{Vision.} 
% % To examine the discriminative performance gap of image understanding models across different difficulty levels, 
% We similarly construct hard and easy negatives in the image space to evaluate image understanding models \footnote{Constructing moderately hard negatives in the image space is not feasible without reliable image editing tool.\lindsey{not very confident about this reason, maybe we should just remove it. @nouha}}. \textbf{i) Hard negative}: a negative image that is generated based on the same text prompt as the positive image, such that it is semantically close to the text prompt, but contains subtle mistakes.
% % identifiable by humans. 
% % We  use AMT to verify the feasibility of these hard negative samples and only retain the ones with agreeable judgments among 3 workers. 
% \textbf{ii) Easy negative}: a negative image that is randomly sampled from the successful generations of a different prompt in the same dataset (as the positive image), such that it is semantically distant from the positive image and can be easily distinguishable.  
% In this setting, the negative image would be semantically distant from the positive image, and hence can be easily distinguishable. 



% For the discriminative setting, we take the subset of text prompts that Midjourney have at least one successful generation, and construct the candidate pairs with a successful generation and a failed generation. \nouha{We don't need to discuss details on how we construct candidates here, this can be move to appendix. We can just mention the overall task. }
% In real user scenario of image generation models, the image selection step, which requires understanding on the generated images, is usually conducted by human.   We consider \textbf{CLIP}~\cite{} and \textbf{Open-CLIP}~\cite{} models for discriminative evaluation, as they are trained to measure the similarity between image and text, and test whether manual image selection can be replaced by image understanding models.  Here, Similarly, we report accuracy as the evaluation metric for the discriminative setting. 

\begin{figure}[t]
   \begin{minipage}[t]{0.4\textwidth}
     \centering
%\includegraphics[width=\linewidth]{figures/exp_mul/average_frequency_of_subgraph_in_training_data.png}
\includegraphics[width=\linewidth]{figures/language/gpt4_disc_gen-cropped.pdf}
\vspace{-22pt}
\caption{\small \gptfour vs. Humans. Humans show a larger positive correlation between their discrimination and generation abilities compared to \gptfour. %\ben{What do the shaded areas inside the dotted lines represent?}
}
\label{fig:gpt4_disc_gen_v2}
   \end{minipage}
   \hfill 
   \vspace{3mm} 
      \begin{minipage}[t]{0.5\textwidth}
     \centering
%\includegraphics[width=\linewidth]{figures/exp_mul/error_type.pdf}
%\includegraphics[width=0.9\linewidth]{tmp_figures/figure 5 thinner.pdf}
\includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}

\caption{\small Quality scores of human-generated responses vs. GPT4 response scores}



%Each curve represents the ratio of \textit{all} nodes appearing at the $i$-th layer of some ground-truth computation graph that belong to a specific category. 
%This ratio is taken over all computation graphs up to \mel{ASK XIMING}. \nouha{remove in-distribution, ood, and replace those with the puzzzle.}
\label{fig:human_gpt4_comparative}
   \end{minipage}
   \vspace{-7mm}
\end{figure}



\subsection{Models' generations are preferred over Humans generations}
To better understand the gap between humans and LLMs, we asked AMT workers to provide their preferences between machine-generated and humans-generated answers in the language-related tasks, along with a rationale behind their choices.\footnote{See Appendix \ref{app:human_eval_details} for details.} While both sets of responses score high in correctness (see Figure~\ref{fig:chatgpt_exp1_language}), Figure~\ref{fig:human_gpt4_comparative} illustrates a notable trend: workers often favor responses from \gptfour over those generated by humans. The same applies for \chatgpt (see Figure~\ref{fig:chatgpt_comparative_v2} in Appendix \ref{app_comparative study}). The rationales provided by humans often indicate a preference for \gptfour due to its responses being longer in length, possessing a more elegant writing style, and being more informative, while human choice is preferred for its brevity and conciseness (Figure~\ref{fig:gpt4_breakdown}). This aligns with the observations made in vision experiments (\S\ref{sec:exp1}), suggesting that 
impressiveness of model generation in human eyes may 
%models' impressiveness to humans may 
rely more on aspects like style than on actual accuracy or understanding of the content.
This preference for model-generated content is intriguing, considering that LLMs may not possess the same level of genuine understanding and selective accuracy as humans, raising questions about the underlying reasons for these preferences.

% \begin{table}[t!]
%     \centering
%   \footnotesize
%     \input{tables/exp1_results}
%      \caption{Caption:  \liwei{working on a plot on this. To be done by EOD Sept 22}}
%     \label{tab:my_label}
% \end{table}






% \begin{table}[t!]
%     \centering
%   \footnotesize
   
% \begin{tabular}{ |p{2cm}||p{1.5cm}|p{2cm}| p{2cm} | p{2cm} |}
%  \hline
% Dataset & Model & Candidate type & Model Disc Accuracy & Human Disc Accuracy\\
% \hline
% \multirow{6}{*}{FaithDial}  & \multirow{3}{*}{GPT4} & hard & 0.63 & 0.86 \\
%  & & med & 0.65 & 0.91  \\
%  & & easy & 0.73 & 1 \\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.60 & same as GPT4 \\
%  & & med & 0.66 &  idem \\
%  & & easy & 0.71 &  idem \\ 
% \hline
% \multirow{6}{*}{Topioca}  & \multirow{3}{*}{GPT4} & hard & 0.92 & 0.91 \\
%  & & med & 0.95 & 0.92  \\
%  & & easy & 0.99 & 0.99 \\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.88 & same as GPT4 \\
%  & & med & 0.92 &  idem \\
%  & & easy & 0.98 &  idem \\ 
% \hline
% \multirow{6}{*}{XSUM}  & \multirow{3}{*}{GPT4} & hard & 0.19 & 0.84\\
%  & & med & 0.82 & 0.88 \\
%  & & easy & 0.99 & 0.98\\ 
%  \cline{2-5}
%  & \multirow{3}{*}{ChatGPT} & hard & 0.10& same as GPT4 \\
%  & & med & 0.82 &  idem \\
%  & & easy & 1.00 &  idem \\ 
% \hline

%  \end{tabular}
%  \caption{Ablation: measuring the effect of the hardness of the candidates on the performance of the models and humans. }
%     \label{tab:negative_candi_results}
% \end{table}

 

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/language/agreement_gpt4-cropped.pdf}
% \caption{Agreement and disagreement between generative and discriminative performance. \liwei{working on refining the plot on this. To be done by EOD Sept 22}}
% \label{fig:agreement}
% % \vspace{-8pt}
% \end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/matrix.png}
% \caption{Agreement and disagreement between generative and discriminative performance (XSUM).}
% \label{fig:agreement}
% % \vspace{-8pt}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/chatgpt_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigure to include them together}}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/language/comparative_gpt4-cropped.pdf}
% \caption{GPT4 vs Human comparative study.}
% \label{fig:human_comparative_study}
% % \vspace{-8pt}
% \end{figure}



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/human_comparative.png}
% \caption{Human comparative study. \nouha{Will improve these plots, but we can see now across all language tasks that humans tend to prefer machine generated answers for both GPT4 and ChatGPT.}}
% \label{fig:human_comparative_study}
% % \vspace{-8pt}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/gpt4_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigures to include them together. We can also separate by task categories} \faeze{the gap decreases as models get stronger}}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/chatgpt_gen_vs_disc.pdf}
%     \caption{\faeze{will make these smaller and do subfigure to include them together}}
%     \label{fig:enter-label}
% \end{figure}


% \begin{table*}[t]
% \scriptsize
% \centering
% \begin{tabular}{l | l  l  l | l }
%  \toprule

%   \bottomrule
% \end{tabular}
% \caption{\small Human Generation quality vs Machine generation quality}
% \label{tab:human_eval}
% \end{table*}






% \subsection{Models Can’t Explain their Own Generations}
% \section{Probing Models' Understanding of their Generations} 
\section{Can Models Understand What They Generate?}
\label{sec:exp2}

% \peter{May want to swtich the word ``probe'' to avoid other associations/existing definitions. Or possibly change sec title to match \S3? e.g. Can AI understand model generations?}

% \faeze{to be consistent with the question-style of sect 3 and Pang wei's suggestion, we can also have this as: "Can Model Understand what it Generates?"} 

%\ake{Based on new framing as discussed earlier, transition now something like ``In the previous section we formulated understanding as ability to select among a space of possible answers for a task, by contrast to ability to generate a single correct answer. In this section, we take a different angle on understanding: given a generated output, can models accurately answer questions about (the content, appropriateness, etc) of that output?'' (Peter refine to make consistent)}


% \begin{figure}[t!]
% \captionsetup[subfloat]{farskip=1pt,captionskip=2pt}
% \centering
%    \subfloat[\small{GPT-4 performance on generation and question answering based on its own output, versus human’s performance on question  answering based on GPT-4’s output.}]{
%       \includegraphics[width = 0.45\columnwidth]{figures/language/interrogative_exp2_gpt4.pdf}\label{fig:lang-expt2-main-results}
%    }\hfill
%    \subfloat[\small{Model versus human performance on
% visual question answering based on generated images}]{
%       \includegraphics[width = 0.485 \columnwidth]{figures/vision/vision_exp1_v3.png}\label{fig:vision-expt2-main-results}
%    }
%    \vspace{-5pt}
%    \caption{
%     \small{ Results on cyclic evaluation.}
%    }
%     \vspace{-10pt}
%     \label{fig:exp2-cyclic}
% \end{figure}

In the previous section, we show that models often excel at generating accurate answers while lagging behind humans in the discriminative task.
%terms of discriminating answers. % \ake{update that conclusion phrasing if needed for latest version of prior section} \nouha{this is valid only for language}. % In this section, we investigate how models struggle \faeze{this is not true about collie which is very constrained gen task} to provide meaningful understanding of their own generation. 
Now we investigate to what extent models can demonstrate meaningful understanding of their own generations---something humans are highly capable of---by directly asking models questions about their generated content in an \emph{interrogative} setup as defined in \S\ref{sec:2}.  %We probe models under two different settings: \textbf{(i) cyclic evaluation} (\S \ref{cyclic_probe})  \textbf{(ii) self-reflection} (\S \ref{self_reflect}). Next, we describe each probing setting in detail.  
%comprising two steps:

% \peter{Reorganizing below, but saved previous version in ``history'' folder}

\paragraph{Language Experimental Setup}

In language, we consider 2 generation settings: \emph{open-ended} where models have loose semantic prompts for generation, and \emph{constrained} where models have \jena{are given?} hard lexical prompts for generation. In both cases, we examine models' understanding of their own generations by asking questions about information from the prompt.



For the \emph{open-ended setting}, we first prompt models to generate a paragraph taking into account some background information. Then using the generation as context, we ask the model multiple-choice questions based on this information,
For example, for \textbf{XSUM} \citep{narayan-etal-2018-dont} (summarization)  we prompt the model to generate an article based on a ground-truth summary, and then ask the model to select the best summary for the generated article. \peter{what are the distractors?} \ximing{same with the ones in exp1} For \textbf{Mutual}$^+$ \citep{cui-etal-2020-mutual} (dialogue), the model generates the conversation history that leads to a given dialogue, and then is asked to choose the best dialogue continuing that history. In \textbf{HellaSwag} \citep{zellers-etal-2019-hellaswag} (commonsense), the model generates the context preceding a given sentence and then selects the most fitting continuation for that generated context.
We report the model generation performance, the selection performance based on content generated by the model, and human selection performance using the model's generated content. %\ake{We should explain lack of human generation results.}. 
We use zero-shot \chatgpt and \gptfour for all the evaluations. 
%\ake{I think we need to give a clearer argument for why asking the model to choose the better generation is a test of understanding?} 
In effect, we are asking the model to use its own generation to answer simple contextual questions of preference \jena{preference? that gets at the content of the generated material?}. As an implicit baseline, we assume humans can answer such questions about their own generations with high accuracy, and so refrain from the complex process of eliciting these generation.

In the \emph{constrained} setting, we use a compositional task that covers diverse generation levels, i.e., word, sentence, paragraph, and passage: \textsc{Collie}-v1 \citep{yao2023collie} \ben{Maybe bold this rather than sc for consistency with other datasets?}, which contains 2,080 constraint instances across 13 different task types shown in Appendix Table \ref{tab:collie_examples}. 
%\faeze{Given the table goes to appendix do you think we need to give an example of the task in this paragraph? or can it wait to next parag} \peter{I think it's fine for now. Maybe in the final version we can give more info}
We zero-shot prompt \chatgpt and \gptfour to generate outputs for 50 examples per task. We then ask models about their generations, specifically whether they satisfy the given constraints. 

\paragraph{Vision Experimental Setup}


\footnotetext{We report the best results on BLIP-2 (\texttt{BLIP2-flan-t5-xxl}), more results can be found in \S\ref{}.}

% \lindsey{Either we can change the title of the subsection, or move the vision paragraph to be a standalone subsection to the end of section 4.} 
We conduct interrogative evaluation on image understanding models via visual question answering in an open-ended setting. We consider \textbf{TIFAv1.0}~\citep{hu2023tifa} as the evaluation benchmark with text prompts from \textbf{COCO}, \textbf{PaintSkill}, \textbf{DrawBench} and \textbf{Parti}~\citep{yu2022scaling}. 
% Based on the text prompt, 
TIFAv1.0 includes questions automatically generated by a language model, only concerning the content specified in the text prompt (\textit{e.g.}, about existence/attributes of an object and relative position between objects). We first ask Midjourney to generate images, based on the text prompts.  Then, we interrogate the understanding models (\textit{e.g.}, BLIP-2)
% (\textit{i.e.}, BLIP-2, BingChat and Bard) 
with questions about the images. AMT is used to collect human responses, and judge the correctness of human/model outputs. 


\subsection{Self-understanding of Generation in Models}


%\input{figures/lang-expt2-main-results}
\paragraph{Language}

\input{figures/lang-expt2-main-results}
Results for the open-ended setting are shown in Figure \ref{fig:lang-expt2-main-results}. 
We observe that while the models excel at generation, they make frequent errors in answering questions about their own generation, indicating a lack of understanding.
%\ake{``Models' discriminative accuracy on their own generations also frequently falls short of humans' accuracy, consistent with ( prev section)''} 
Humans, who could not generate such text at the same speed or scale, consistently achieve higher accuracy in QA compared to the model, though questions are about the model's own output.
%The model's performance is also consistently lower than human's performance when answering questions based model's generation. 
%Noticeably, the model's understanding on model's generation  consistently lags behind human's understanding on model's generation desipte that model has the advantage that questions are based on its own generation.
%The model's performance consistently lags behind that of humans when answering questions based on its own generated content. 
We note that the humans in this study are not experts; producing text as sophisticated as the model's output could be a significant challenge. We anticipate that the performance gap in understanding one's own generation would widen even more when comparing the model to human experts, who are likely to answer questions about their own generations with near-perfect accuracy.




Next, the constrained setting: Figure \ref{fig:gpt4_collie_condensed} shows \gptfour's constraint satisfaction rate across 3 representative tasks in Collie (see Figure \ref{fig:collie_gpt4_full} for full results). Certain tasks with simple constraints such as \texttt{word01} (generating a word with a minimum number of letters), and \texttt{sent04} (generating a sentence containing three specific words) are less challenging for models. %, and \texttt{para01} (generating a paragraph with each sentence starting with word A) are less challenging for models. 
However, we observe a significant drop in performance when posed with arbitrary position constraints and strict counting requirements (e.g., \texttt{sent02}, generating a sentence with x words, where the 3rd word is A, and the 7th word is B, ...), suggesting that current models cannot handle generations when faced with rich compositional constraints. Unlike the open-ended setting, we find models are often better at answering questions about their generations than generating. We propose that more precise constraints like this are easier to judge (trivial for humans) while being much harder for models to exercise flexible generation over.
\input{figures/collie_condensed_v2}





\paragraph{Vision}


\begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-5pt}
\centering
% \includegraphics[width=\linewidth]{figures/language/interrogative_exp2_vertical.pdf}
\includegraphics[width=\linewidth]{figures/vision/vision_exp1_v3.png}
% \vspace{-15pt}
\caption{\small{Model versus human performance on visual question answering based on generated images.\footnotemark}}
% \vspace{-26pt}
\label{fig:vision-expt2-main-results}
\end{wrapfigure}
Figure~\ref{fig:vision-expt2-main-results} shows that image understanding models still fall short of human accuracy in answering \textit{simple} questions about elements in the generated images. At the same time, state-of-the-art image generation models can generate images at a quality and speed beyond most humans, \peter{Cite some support}%\ake{presented here as is, the reader may be confused because the results themselves don't actually show anything about models' generations as compared to humans}
indicating a relative gap between generation (stronger) and understanding (weaker) in vision AI compared to humans. 
%\lindsey{Note that though we are not testing the same model on both generation and understanding for vision modality, we still arrive at a similar conclusion to the language domain, that is models do not have full understanding about models' generation.}
%\lindsey{I added my original sentence back, which may avoid mentioning any assumption about human generation.}
% \peter{tried to handle this. My sentence still needs some work to be convincing}
Surprisingly, the performance gap between models and humans is smaller for simpler models than advanced multimodal LLMs (\textit{i.e.}, Bard and BingChat), which have some visual understanding, but still struggle to answer simple questions about generated images.







% \begin{figure}[th]
%     \centering
% \includegraphics[scale=0.3]{figures/generative_collie.pdf}
%     \caption{Constraint Satisfaction of GPT-3.5 (left) and GPT-4 (right) Generations on Collie Benchmark \cite{}.}
%     \label{fig:gen_collie}
% \end{figure}

% \begin{figure}[th]
%     \centering
% \includegraphics[scale=0.25]{figures/discriminative_collie_v2.pdf}
%     \caption{Accuracy of GPT-3.5 (left) and GPT-4 (right) on understanding the correctness of their own generations.
%     }
%     \label{fig:disc_colllie}
% \end{figure}


\input{figures/disagreement_figure}


==> sections/history/4_discussion_v0.tex <==
\section{Discussion}
\subsection{Assessing the generative AI paradox}

\peter{Quick, key-point discussion of where the experiments support the paradox, and where it is more complicated. Make the simple case that any significant divergence from humans supports paradox idea. No more than a couple of paragraphs.}

\subsection{Proposed explanations and points of future study}
\label{subsec:discussion-why}
Given the above evidence in support of the Generative AI Paradox, the next question is: \emph{what factors could lead to models excelling at generation even when they cannot demonstrate strong understanding?} We propose some hypotheses below, and encourage future work to explore this question.



\paragraph{Task Openness} Our results suggest that the \emph{openness} of tasks (i.e. how much freedom there is in providing correct responses) is correlated with the gap between generation and discrimination in models (REF). One possibility is that open tasks leave more flexibility for models to fall back on memorized data and confidence regions, whereas closed tasks force specific answer, causing models to expose gaps in knowledge, similar to discriminative tasks. %\peter{Cite the "A is B" paper? I have thoughts on this }

%While we aim to only highlight the Generation Paradox, we do conjecture about certain features of these large models which could be contributing to this difference in skills between models and humans.  

\paragraph{Underlying Generative Objective} Generative models are defined by the generative learning objective, which explicitly encourages reconstruction and generation of the training data/distribution, while only implicitly encouraging understanding insofar as it assists this goal. Human learning likely has objectives besides pure reconstruction of stimuli, for instance interaction-based goals \citep{bisk-etal-2020-experience}, which would lead to divergent behavior. \peter{probably the wrong ref}

%\paragraph{Underlying Generative Objective}
%Most models are trained explicitly (and intensively) for generation, so they are designed to excel at it.  For example, the objective function used to train LLMs minimizes error in next-word prediction and hence focuses only on the models' capacity to generate fluent, likely language. Since the objective function has a single goal of generation, it naturally results in the model's exceptional generation ability. Secondly, the training objective trains the model to reconstruct every data point in the training dataset. Therefore, the model is more aligned to a generation task, which allows it to rely on these reconstructions to piece together an appropriate response \cite{raven} rather than analyzing and distilling meaning from many training samples to identify one correct solution. In contrast to this simple, one objective optimization, humans language construction is rather complex, involving multiple brain regions \cite{Walenski} and might be more compared to the process of multiple revisions rather than next-token constructions \cite{Friederici}.

% \peter{Ideas:}
% \begin{itemize}
%     \item Models is trained explicitly to generate (objective function)
%     \item And trained to reconstruct every data point it sees (for traditional LM, and for image models)
%     \item We know intuitively that the human objective is not this. Although we don't know the human learning objective, theories say ...
%     \item Also, signal is quite a bit more dense for generation than for understanding. It makes sense that strongest representations will be generative because it uses all info in training data, but also that these representations will be generation-focused. 
    % \item and possibly put forward a more concrete hypothesis of what's going on. E.g. models are able to use simpler composition of more complex/esoteric pieces than humans. So a lot of work is kind of ``precomputed'' in terms of being memorized, and models simply need to stitch these more complicated things together, rather than reason through any of them
% \end{itemize}

\paragraph{Training Data}
Many large models are trained by making multiple passes through huge swaths of internet data, while it would take an average human reader over 32 years to simply read all the pages of Wikipedia \cite{Wikipedia_num_words,BRYSBAERT2019104047}. This obvious discrepancy in not only quantity, but also diversity of knowledge is likely to encourage models to use existing solutions to problems, which they have already seen, whereas humans have not and therefore need to exercise understanding and reasoning to answer the same questions.


% \peter{Ideas:}
% - Humans read on average 238 words/min for non-fiction and 260 words/min for fiction --> average is 249 words/min
% - Currently 4.3billion words on wikipedia as of Sept. 22nd
    % \item \textbf{Knowledge access}: LMs possess unique advantages over humans when it comes to knowledge access and generation capabilities. LMs have been trained on vast and diverse datasets, encompassing a wide range of topics and domains. This gives them access to information that is not only extensive but also highly specialized. In contrast,  humans have limitations in terms of the breadth and depth of their knowledge. No single human can be an expert in all areas, whereas LMs can generate content on any topic.
        % \begin{enumerate}
        %     \item \textbf{Memory and Recall}: LMs do not suffer from the limitations of human memory and recall. They can recall specific details and facts with high precision, even if those details were mentioned deep within their training data. Humans, on the other hand, often struggle with forgetting or misremembering information, and they may not always have access to comprehensive reference materials. LMs are consistent in their knowledge and information recall. They don't get tired, distracted, or biased by emotions, which can affect the accuracy and consistency of human knowledge. 
        %     \item 
        % \end{enumerate}

\paragraph{Memorization and Knowledge} A related factor is memorization of data, objects, and knowledge from the training set, e.g. recent work shows that language models memorize a significant portion of training data (CITE). \peter{more here}

\paragraph{Development Pressures} Evolutionary and economic pressures can affect the way that AI technologies develop. For instance, popular language model architectures have been found to have a preference for languages like English \citep{Ravfogel2019StudyingTI} which has seen the most attention in NLP (CITE) and thus the most reward for improvement. It is feasible that similar pressures would encourage architectures, training paradigms, and other decisions that favor improving generation over understanding, as generation is harder for humans and thus more useful/valuable behavior. 


%\peter{Ideas:}

\paragraph{Modeling of a medium}

Another key distinction for generative models is that they are modeling a \emph{medium} rather than an \emph{individual} (e.g. a human), although we often query them as if they were individuals. \citep{andreasnaacl}. For example, language models are trained over documents from many authors. While context may allow models to get closer to emulating a specific individual, models may still tend towards behavior that looks \emph{distributionally correct} rather than \emph{individually correct}, prioritizing stylistic and document-wide features rather than details that are probed more extensively in understanding tasks. In any case, this is a significant difference from humans. \peter{mention our stylistic results here}


\subsection{Limitations and Implications}

Finally, we discuss limitations of this work and implications for future work.

One possible limitation is dataset contamination. For example, GPT-4 and ChatGPT may have been exposed to existing benchmarks at training time (CITE). However, we argue that this should have similar affects on both generation \emph{and} discriminative evaluation in \S\ref{} (exp 1) as both use the same model inputs. Further, our evaluations in (exp 2) use a novel setup which is based on generation and so would not have been seen at training time \peter{CHECK THIS}.

We also focus on small a set of the most popular/widely used models. Future work should investigate a wider range of models, including smaller and weaker models, for which we hypothesize the paradox may be even more pronounced (CITE COMPARISON BETWEEN CHATGPT AND GPT4). Factors like memorization, influenced by training paradigm, likely have an effect as well.

While our evaluation of human performance is focused, future work can explore more extensive and explicit comparisons between model and human performance. We also advocate for adopting comparison to humans as a widespread practice, to carefully judge when model capabilities extrapolate the same way as human capabilities, and when they do not. 

Finally, we only investigate \emph{one} divergence between humans and models here. Proposing and testing other points of divergence in the curvature of artificial and natural intelligence exceeds our scope but will be imperative to calm concerns and calibrate excitement. 





%\peter{ideas:}
%\begin{itemize}
%    \item Dataset contamination (although this may only reduce the paradox...)
%    \item limited models and modalities (e.g. what about smaller models, how does this change over time?)
%    \item More extensive human analysis needed. and generally, comparison with human is more important than ever
%    \item We are only investigating \emph{one gap} here, but there are lots of curvature questions
%\end{itemize}






==> sections/history/4_discussion_v1.tex <==
\section{Discussion}
\subsection{Assessing the generative AI paradox}

\peter{Quick, key-point discussion of where the experiments support the paradox, and where it is more complicated. Make the simple case that any significant divergence from humans supports paradox idea. No more than a couple of paragraphs.}

\subsection{Proposed explanations and points of future study}
\label{subsec:discussion-why}
Given the above evidence in support of the Generative AI Paradox, the next question is: \emph{what factors could lead to models excelling at generation even when they cannot demonstrate strong understanding?} We propose some hypotheses below, and encourage future work to explore this question.

\textbf{Task Openness} Our results suggest that the \emph{openness} of tasks (i.e. freedom in output space) is correlated with the gap between generation and discrimination in models (REF). One possibility is that open tasks leave more flexibility for models to fall back on memorized data and confidence regions, whereas closed tasks force specific answer, causing models to expose gaps in knowledge, similar to discriminative tasks.

\textbf{Underlying Generative Objective} Generative models are defined by the generative learning objective, which explicitly encourages reconstruction and generation of the training data/distribution, while only implicitly encouraging understanding insofar as it assists this goal. Human learning likely has objectives besides pure reconstruction of stimuli, for instance interaction-based goals \citep{bisk-etal-2020-experience}, which would lead to divergent behavior. \peter{probably the wrong ref}

\textbf{Training Data}
Many large models are trained by making multiple passes through huge swaths of internet data, while it would take an average human reader over 32 years to simply read all the pages of Wikipedia \cite{Wikipedia_num_words,BRYSBAERT2019104047}. This obvious discrepancy in not only quantity, but also diversity of knowledge is likely to encourage models to use existing solutions to problems, which they have already seen, whereas humans have not and therefore need to exercise understanding and reasoning to answer the same questions.

% \textbf{Memorization and Knowledge} A related factor is memorization of data, objects, and knowledge from the training set, e.g. recent work shows that language models memorize a significant portion of training data (CITE). \peter{more here}
    
\textbf{Development Pressures} Evolutionary and economic pressures can affect the way that AI technologies develop. For instance, popular language model architectures have been found to have a preference for languages like English \citep{Ravfogel2019StudyingTI} which has seen the most attention in NLP (CITE) and thus the most reward for improvement. It is feasible that similar pressures would encourage architectures, training paradigms, and other decisions that favor improving generation over understanding, as generation is harder for humans and thus more useful/valuable behavior. 

\textbf{Modeling of a medium}
    Another key distinction for generative models is that they are modeling a \emph{medium} rather than an \emph{individual} (e.g. a human), although we often query them as if they were individuals. \citep{andreasnaacl}. For example, language models are trained over documents from many authors. While context may allow models to get closer to emulating a specific individual, models may still tend towards behavior that looks \emph{distributionally correct} rather than \emph{individually correct}, prioritizing stylistic and document-wide features rather than details that are probed more extensively in understanding tasks. In any case, this is a significant difference from humans. \peter{mention our stylistic results here}



\subsection{Limitations and Implications}

Finally, we discuss limitations of this work and implications for future work.

One possible limitation is dataset contamination. For example, GPT-4 and ChatGPT may have been exposed to existing benchmarks at training time (CITE). However, we argue that this should have similar affects on both generation \emph{and} discriminative evaluation in \S\ref{} (exp 1) as both use the same model inputs. Further, our evaluations in (exp 2) use a novel setup which is based on generation and so would not have been seen at training time \peter{CHECK THIS}.

We also focus on small a set of the most popular/widely used models. Future work should investigate a wider range of models, including smaller and weaker models, for which we hypothesize the paradox may be even more pronounced (CITE COMPARISON BETWEEN CHATGPT AND GPT4). Factors like memorization, influenced by training paradigm, likely have an effect as well.

While our evaluation of human performance is focused, future work can explore more extensive and explicit comparisons between model and human performance. We also advocate for adopting comparison to humans as a widespread practice, to carefully judge when model capabilities extrapolate the same way as human capabilities, and when they do not. 

Finally, we only investigate \emph{one} divergence between humans and models here. Proposing and testing other points of divergence in the curvature of artificial and natural intelligence exceeds our scope but will be imperative to calm concerns and calibrate excitement. 





%\peter{ideas:}
%\begin{itemize}
%    \item Dataset contamination (although this may only reduce the paradox...)
%    \item limited models and modalities (e.g. what about smaller models, how does this change over time?)
%    \item More extensive human analysis needed. and generally, comparison with human is more important than ever
%    \item We are only investigating \emph{one gap} here, but there are lots of curvature questions
%\end{itemize}






==> sections/history/7_related_work_v0.tex <==
\section{Related Work}
% \lasha{ working on this section under progress}

% \peter{This paper seems quite relevant} \cite{Berglund2023TheRC} Abhilasha: thanks, added!




\paragraph{Paradoxes in Large Language Model Behavior}

Prior work has employed large language models to \emph{improve their own generations}, finding that models can successfully identify mistakes (despite these mistakes being generated by the models themselves). We consider this a type of paradoxical behavior: if models can easily identify mistakes in their own generations, then why do models generate those errors to begin with? \cite{madaan2023self} prompt models to critique their own generations, and then prompts models to improve their previous generation given the critique. \cite{agrawal2023language} find that models can effectively identify hallucinated content in their own generations when prompted. \cite{gero2023self} find that in clinical information extraction tasks, models are able to identify elements that are erroneously omitted in their original generations, as well as inaccurate statements in their own generations.  

\paragraph{Inconsistency in Large Language Models}

Considerable prior work suggests that large language models do not demonstrate behavior that corresponds to a robust representation of concepts. For example, \cite{kassner2020negated} and \cite{Ettinger_2020} find that models will generate correct facts but also their negations. \cite{elazar-etal-2021-measuring} and \cite{ravichander-etal-2020-systematicity} demonstrate that language models make inconsistent predictions when prompted with paraphrases or entailed statements. \cite{ribeiro-etal-2019-red} study consistency in question-answering systems, finding that generated answers often contradict each other. \cite{jang-etal-2022-becel} construct a benchmark for measuring behavioral (in)consistency, finding that large language models often make inconsistent predictions. \cite{Berglund2023TheRC} describe ''inconsistent knowledge'' in large language models, where models may correctly recognize factual knowledge which was explicitly stated in their training data, but fail to make inferences related to those facts. Our work ties into these lines of inquiry seeking to shed light on the fundamental limitations of large language models. We demonstrate that competence at generation does not entail understanding ability even for state-of-the-art models. 

\paragraph{Large language models and human cognitive mechanisms}
While the exact mechanisms that language models use to address natural language tasks remains an open research question, prior work has investigated if models possess similar competencies to humans at all. \cite{stojnic2023commonsense} evaluate commonsense psychology in models and humans--- finding that while infants can reason about the causes of actions by an agent, models are not capable of emulating infants' knowledge. Similarly, \cite{sap2022neural} examine Theory-of-Mind in large language models, showing that language models fail to demonstrate this kind of social intelligence. Similarly, \cite{storks-etal-2021-tiered-reasoning, bisk2020piqa} study physical commonsense reasoning in large language models and find considerable discrepancies between human and model capacities. Our work continues this line of enquiry, shedding light on the vastly different abilities of models compared to humans when it comes to generating and understanding language.




% \paragraph{}

==> sections/vision_exp2.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/vision/vision_exp2_v2.png}
%     % \vspace{-15pt}
%     \caption{\small {Model versus human performance on visual question answering based on generated images.\footnotemark}}
%     \label{fig:vision-expt2-main-results}
%     \vspace{-20pt}
% \end{figure}

\begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-5pt}
\centering
% \includegraphics[width=\linewidth]{figures/language/interrogative_exp2_vertical.pdf}
\includegraphics[width=\linewidth]{figures/vision/vision_exp1_v3.png}
% \vspace{-15pt}
\caption{\small{Model versus human performance on visual question answering based on generated images.\footnotemark}}
% \vspace{-26pt}
\label{fig:vision-expt2-main-results}
\end{wrapfigure}

\footnotetext{We report the best results on BLIP-2 (\texttt{BLIP2-flan-t5-xxl}), more results can be found in \S\ref{}.}

\paragraph{Vision} 
% \lindsey{Either we can change the title of the subsection, or move the vision paragraph to be a standalone subsection to the end of section 4.} 
We conduct interrogative evaluation on image understanding models via visual question answering in an open-ended setting. We consider \textbf{TIFAv1.0}~\citep{hu2023tifa} as the evaluation benchmark, with text prompts from \textbf{COCO}, \textbf{PaintSkill}, \textbf{DrawBench} and \textbf{Parti}~\citep{yu2022scaling}. 
% Based on the text prompt, 
TIFAv1.0 includes questions automatically generated by a language model, only concerning the content specified in the text prompt (\textit{e.g.}, about existence/attributes of an object and relative position between objects). We first ask Midjourney to generate images, based on the text prompts.  Then, we interrogate the understanding models (\textit{e.g.}, BLIP-2)
% (\textit{i.e.}, BLIP-2, BingChat and Bard) 
with questions about the images. AMT is used to collect human responses, and judge the correctness of human/model outputs. 
% \faeze{Lindsey, can we skip the part after "Note that..." to save space? $\rightarrow$}\lindsey{yes!} 
% Note that, even when the generated image does not strictly match the text prompt, we can still probe both models and humans for their understanding, with questions that are answerable given the image. \ake{This sounds different from the language experiments above, where models were asked to choose the best generation, whereas this is asking actual questions about the generated content?}\lindsey{yes, the setup is different for vision. we are using VQA for this experiment. But in the same spirit that we ask generation model to generate image based on the task to probe the understanding model.}

Figure~\ref{fig:vision-expt2-main-results} shows that image understanding models still fall short of human accuracy in answering \textit{simple} questions about elements in the generated images. At the same time, state-of-the-art image generation models can generate images at a quality and speed beyond most humans \ake{presented here as is, the reader may be confused because the results themselves don't actually show anything about models' generations as compared to humans}, indicating a gap between generation and understanding in vision AI. 
\lindsey{Note that though we are not testing the same model on both generation and understanding for vision modality, we still arrive at a similar conclusion to the language domain, that is models do not have full understanding about models' generation.}
\lindsey{I added my original sentence back, which may avoid mentioning any assumption about human generation.}
% \peter{tried to handle this. My sentence still needs some work to be convincing}
Surprisingly, the performance gap between models and humans grows from simpler models to advanced multimodal LLMs (\textit{i.e.}, Bard and BingChat), which have shown intriguing properties in visual understanding, but still struggle to answer simple questions about generated images. %\lindsey{For the last part, I am trying to say that even with the strong visual understanding capabilities shown by GPT-4V (behind BingChat), we still observe generative AI paradox, that model is better at generation, while worse in understanding, compared to human.}  \peter{could you elaborate a little more? Sentence says ``even bigger for more advanced'' and I'm not sure I totally understand although probably just missing something}\lindsey{oh, in figure 9, we are seeing bigger gaps between bard/bingchat and human, than BLIP2 and human, so was trying to say something about that. people may have the impression that bard and bingchat are stronger multimodal models, but our results suggest they actually fail more easily in terms of this interrogative evaluation.}

% \lindsey{Nouha and I had a discussion about how to fit vision exp 2 into this section. we can probably frame it in the same way as cyclic evaluation. though the cycle does not go back to the same model, it still go back to a model. the flow of vision exp 2 is: (1) text prompt $\rightarrow$ QA, (2) text $\rightarrow$ generation model $\rightarrow$ image, (3) image + Q $\rightarrow$ understanding model $\rightarrow$ A. wdyt?}\faeze{Yes this sounds good. Ximing's version due to having a single model is: (1) instruction + A $\rightarrow$ paragraph, (2) paragraph + Q $\rightarrow$ A}

% \nouha{The conclusion will be a bit different from language in the sense, we're not testing the model on their own generations but we're showing the gap between the models' impressive image generation and their  understanding when asked questions about the images. We're also contrasting this performance to humans. }
% \lindsey{Per Yejin's suggestion, we can consider moving  vision experiment  to the end of 4.3. Will draft something today.}

==> tables/exp1_results.tex <==
%%% Consensing the table

% \begin{table}[t!]
%     \centering
%   \footnotesize
   
\begin{tabular}{ |p{2cm}||p{1.5cm}|p{1cm}| p{1cm} | p{1cm} | p{1cm} | p{1cm} |}
 \hline
Domain & Dataset & Model  & Model Gen Acc & Model Disc Acc & Human Discr Accu & Human Gen acc \\
\hline
\multirow{8}{*}{Dialogue} & \multirow{2}{*}{FaithDial}  & {GPT4}  & {0.83} & {0.67} & \multirow{2}{*}{0.86} & \multirow{2}{*}{0.99} \\
 & & {ChatGPT} & 0.89 & 0.65 &  &\\
\cline{2-7}
& \multirow{2}{*}{DREAM} & GPT4  & 0.96 & 0.96 & \multirow{2}{*}{0.96} & \multirow{2}{*}{0.95}\\
 & & ChatGPT  & 0.97 & 0.90 & &\\
\cline{2-7}
& \multirow{2}{*}{Mutual$^+$} & GPT4  & 0.99 & 0.76 & \multirow{2}{*}{0.80} & \multirow{2}{*}{0.79}\\
 & & ChatGPT  & 0.99 & 0.63 & &\\
\hline
\multirow{2}{*}{Conv. QA} & \multirow{2}{*}{Topioca}  &{GPT4}  & 0.93 & 0.95 & \multirow{2}{*}{0.92} & \multirow{2}{*}{0.94}\\
 & & {ChatGPT}  & 0.92 & 0.92 & &\\
\hline
\multirow{2}{*}{QA} & \multirow{2}{*}{RACE} & GPT4  & 0.96 & 0.89 & \multirow{2}{*}{0.86} & \multirow{2}{*}{0.90} \\
 & & ChatGPT  & 0.94 & 0.83 & &\\
\hline
\multirow{2}{*}{Summarization} & \multirow{2}{*}{XSUM} & {GPT4}  & 0.99 & 0.66 & \multirow{2}{*}{0.84} & \multirow{2}{*}{0.88}\\
& & ChatGPT & 0.99  & 0.64 & &\\

\hline
\multirow{10}{*}{Commonsense} & \multirow{2}{*}{CSQA} & GPT4   & 0.96 & 0.87 & \multirow{2}{*}{0.92} & \multirow{2}{*}{0.95}\\
 & & ChatGPT & 0.97 & 0.72 & & \\
\cline{2-7}
& \multirow{2}{*}{SocialIQA} & GPT4 & 0.89 & 0.72 & \multirow{2}{*}{0.87} & \multirow{2}{*}{0.86}\\
 & & ChatGPT  & 0.98 & 0.70 &  &\\
\cline{2-7}
 & \multirow{2}{*}{HellaSwag} & GPT4   & 0.96 & 0.87 & \multirow{2}{*}{0.88} & \multirow{2}{*}{0.94}\\
 & & ChatGPT & 0.85 & 0.79 & &\\
\cline{2-7}
 & \multirow{2}{*}{PIQA} & GPT4   & 0.99 & 0.92 & \multirow{2}{*}{0.92} & \multirow{2}{*}{0.86}\\
 & & ChatGPT  & 0.97 & 0.82 & &\\
\cline{2-7}
& \multirow{2}{*}{$\alpha$NLI/$\alpha$NLG} & GPT4  & 0.97 &  0.80 & \multirow{2}{*}{0.87} & \multirow{2}{*}{0.92}\\
 & & ChatGPT  & 0.91 & 0.70 & &\\
\hline
 
 \multirow{4}{*}{NLI} & \multirow{2}{*}{WaNLI} & GPT4   & 0.73 &  0.63 & \multirow{2}{*}{0.85}& \multirow{2}{*}{0.90}\\
 & & ChatGPT & 0.62 & 0.43 & &\\
 \cline{2-7}
& \multirow{2}{*}{$\delta$-NLI} & GPT4   & 0.89 &  0.92 & \multirow{2}{*}{0.87} & \multirow{2}{*}{0.92}\\
 & & ChatGPT  & 0.85 & 0.75 & &\\
\hline
 \end{tabular}
%  \caption{Caption: \nouha{reporting the hard negative for the discriminative accuracy, will add another table to show the difference between hard and easy. Hard and easy are not applicable for all the tasks, this is why I moved it to a new table.} \faeze{I think having a pot similar to figure \ref{fig:disc_colllie} with their generative vs discriminative performance next to each other is nice and makes the comparison easier. I can do that if you agree on having plots  } \nouha{Good idea, was thinking of that as well. Just having this table now to get a sense of what we have vs not. For each dataset, we can have 1) GPT4/ChatGPT generative vs Human generative (working on running this) and 2) GPT4/ChatGPT discriminative vs Human discriminative) I will add the plots once the experiment is done.}}
%     \label{tab:my_label}
% \end{table}

==> tables/table_of_content.tex <==
% \usepackage{multirow}

\begin{table}[]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|cccccc|c}
\toprule
\multirow{2}{*}{Section} & \multicolumn{2}{c}{Understanding Type} & & \multicolumn{2}{c}{Modality} & \multirow{2}{*}{\thead{Generator is \\ Understander?}} & \multirow{2}{*}{Findings} \\ \cline{2-3} \cline{5-6}
                         & Selective        & Interrogative       & & Language       & Vision      &                                              &                           \\ \hline \cline{1-3} \cline{5-8} 
\S 3.1    &       \cmark           &      \xmark               & &     \cmark        &       \xmark       &                 \cmark                             & Usually                   \\
\S 3.2    &        \xmark         &          \cmark           & &      \cmark        &      \xmark        &                  \cmark                            & Somewhat                  \\
\S 3.3    &         \cmark       &            \xmark         & &        \xmark       &       \cmark      &                     \xmark                         & Complicated               \\
\S 3.4    &      \xmark            &           \cmark          & &        \xmark       &        \cmark     &                      \xmark                        & Somewhat                  \\ \hline
\end{tabular}
\caption{Overview of \faeze{I'm thinking with a clear/brief roadmap we could skip this as well. Let's keep for now tho}
%\peter{Does anyone have thoughts on if we should only have the checkmarks? (and leave other spaces blank) Wondering if the 'x' reads as too negative and possibly unnecessary} \nouha{where do you refer to this table in the text? I find this table somewhat confusing; for example, how do you read the first row? is it for selective mode in language there is often a paradox? I think the red 'x' is so confusing. Depending on the page limit, we might end up moving it to appendix?   }
}
\label{tab:tab-of-content}
\end{table}


% \begin{table}[]
% \begin{tabular}{c|ccccc|c}
% \hline
% \multirow{2}{*}{Section} & \multicolumn{2}{c}{Understanding Type} & \multicolumn{2}{c}{Modality} & \multirow{2}{*}{Generator is Understander/?} & \multirow{2}{*}{Paradox?} \\ \cline{2-5}
%                          & Selective        & Interrogative       & Language       & Vision      &                                              &                           \\ \hline
% \S 3.1    &       \cmark           &      \xmark               &        \cmark        &       \xmark       &                 \cmark                             & Usually                   \\
% \S 3.2    &        \xmark         &          \cmark           &        \cmark        &      \xmark        &                  \cmark                            & Somewhat                  \\
% \S 3.3    &         \cmark       &            \xmark         &         \xmark       &       \cmark      &                     \xmark                         & Complicated               \\
% \S 3.4    &      \xmark            &           \cmark          &         \xmark       &        \cmark     &                      \xmark                        & Somewhat                  \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:tab-of-content}
% \end{table}
